Secure Semantic Communications via AI Defenses: Fundamentals, Solutions, and Future Directions

Semantic communication (SemCom) redefines wireless communication from reproducing symbols to transmitting task-relevant semantics. However, this AI-native architecture also introduces new vulnerabilities, as semantic failures may arise from adversarial perturbations to models, corrupted training data, desynchronized priors, or misaligned inference even when lower-layer transmission reliability and cryptographic protection remain intact. This survey provides a defense-centered and system-oriented synthesis of security in SemCom via AI defense. We analyze AI-centric threat models by consolidating existing studies and organizing attack surfaces across model-level, channel-realizable, knowledge-based, and networked inference vectors. Building on this foundation, we present a structured taxonomy of defense strategies organized by where semantic integrity can be compromised in SemCom systems despite correct symbol delivery, spanning semantic encoding, wireless transmission, knowledge integrity, and coordination among multiple agents. These categories correspond to distinct security failure modes, including representation fragility, channel-realizable manipulation, semantic prior poisoning or desynchronization, and adversarial propagation through distributed inference. We also examine security utility operating envelopes that capture tradeoffs among semantic fidelity, robustness, latency, and energy under realistic constraints, survey evaluation frameworks and representative applications, and identify open challenges in cross-layer composition and deployment-time certification. Overall, this survey offers a unified system-level perspective that enables readers to understand major threat and defense mechanisms in AI-native SemCom systems and to leverage emerging security techniques in the design and deployment of robust SemCom architectures for next-generation intelligent networks.

==> 5_backup.tex <==
\section{How AI Defenses Can Be Used in Semantic Communication Systems} \label{sec:4layered_defense}
As discussed in Section~\ref{sec:AI-security}, the AI-native design of SemCom introduces new threat surfaces. These surfaces allow adversaries to induce semantic failure, leakage, or misalignment without violating syntactic correctness or lower-layer integrity. While the preventive, reactive, and certifiable categories discussed in Section~\ref{sec:AI_security_new} remain conceptually useful, their realization in SemCom is fundamentally system-dependent, shaped by physical channels, shared knowledge, and distributed inference. Safeguarding SemCom, therefore, requires defense mechanisms that extend beyond traditional bit-level reliability and cryptographic protection, and that are explicitly instantiated at the system level. 

In this section, we survey defense foundations for secure SemComs based on AI defense. Rather than treating security as an isolated add-on, we organize defenses according to how and where they intervene in the SemCom pipeline as illustrated in Fig.~\ref{fig:sec4}, bridging model-centric AI security techniques with the architectural realities of SemCom systems. We begin by outlining a defense design philosophy that connects AI security principles with SemCom architectures. We then review defenses at the encoder and decoder, channel, knowledge-base, and network levels, highlighting how these mechanisms compose to provide end-to-end semantic security.


\subsection{Defense Design Philosophy for Semantic Communication} \label{sec:principle}

%Most existing AI defense techniques are developed in a model-centric setting, where the objective is to protect a single learned function $f_\theta : \mathcal{X} \rightarrow \mathcal{Y}$ against adversarial manipulation, data poisoning, or information leakage. SemCom systems, however, embed such models within a broader pipeline that includes semantic encoding and decoding, channel transmission, shared knowledge bases, and network-level coordination. As a result, defenses that are effective for standalone models do not directly translate to SemCom systems without reinterpretation at the system level.

%\textbf{Principle 1: Semantic security is end-to-end.}
%Semantic correctness is determined by the composition of multiple learned and non-learned components rather than by any single model. Protecting an individual semantic encoder or decoder is therefore necessary but insufficient. Semantic failures may arise from channel-realizable perturbations, inconsistencies in shared knowledge, or propagation effects in multi-agent settings. Defense design must explicitly consider where semantic information is formed, transformed, and consumed, and ensure that vulnerabilities at one interface are not amplified downstream.

%\textbf{Principle 2: Defenses should align with both time and location of intervention.}
%Defenses for SemCom can be categorized along two complementary dimensions. The first dimension concerns \emph{when the defense is applied}. Along the temporal dimension, defenses follow the preventive, reactive, and certifiable taxonomy introduced in Section~\ref{sec:IIIC}, but must now be mapped to concrete intervention points within the SemCom pipeline. %Training-time preventive defenses harden semantic models before deployment by shaping representations and learning objectives so that admissible perturbations induce limited semantic distortion. Inference-time defenses operate during system execution, monitoring or mitigating semantic manipulation, often trading latency or coverage for robustness. Certified and verifiable defenses provide formal guarantees under explicit threat models and are most relevant in safety-critical or mission-critical settings.
%Another dimension concerns \emph{where the defense intervenes in the SemCom pipeline}. Encoder- and decoder-level defenses focus on robust representation learning and privacy-aware semantics. Channel-level defenses protect task-level semantic utility under physical constraints. Knowledge-base-level defenses secure shared semantic priors against poisoning, desynchronization, or inference-based leakage. Network-level defenses address emergent threats arising from multi-agent interaction, coordination, and semantic propagation.

%\textbf{Principle 3: Robustness should be semantically efficient.}
%SemCom operates under strict constraints on rate, latency, energy, and computation. Defenses that substantially increase redundancy, model complexity, or inference delay may negate the efficiency gains that motivate SemCom. Effective defense design must therefore prioritize semantic efficiency, achieving the largest reduction in semantic distortion or task degradation per unit of communication or computation cost.

%\textbf{Principle 4: Defenses should support composability across system layers.}
%Rather than relying on a single monolithic safeguard, SemCom systems benefit from layered defenses that operate at different stages of the pipeline. Preventive defenses can reduce attack surfaces early, inference-time mechanisms can trigger adaptation or fallback strategies when manipulation is suspected, and certified components can serve as safety envelopes where failure is unacceptable. This layered view shifts the focus from protecting individual models to safeguarding SemCom systems as integrated pipelines.

Traditional AI defenses focus on protecting individual models, but SemCom systems require a broader, system-level view. Because semantic correctness emerges from interactions among learned models, communication channels, shared knowledge, and network dynamics, security should be treated as an end-to-end property. This shift expands the attack surface beyond isolated models and demands defenses that explicitly account for how semantic information is created, transformed, and propagated across the pipeline.

Table \ref{tab:design_principle} summarizes the four design principles in secure SemCom based on AI defenses. In general, defenses should be aligned with both the timing and location of intervention, respect the efficiency constraints that motivate SemCom, and remain composable across system layers. Rather than replacing existing AI defenses, these principles reinterpret and integrate them into SemCom pipelines, enabling robust protection of shared meaning in adversarial environments.
% -------------------------------------------------

\begin{table*}[t]
\caption{Design Principles for AI Defense in Semantic Communication Systems}
\label{tab:design_principle}
\centering
\renewcommand{\arraystretch}{1.15}
\footnotesize

\begin{tabular}{%
p{2.5cm}   % Principle
p{2.6cm}   % Defense Focus
p{5.0cm}   % Key Observation
p{5.8cm}   % Design Implication
}
\hline
\textbf{Principle} &
\textbf{Defense Focus} &
\textbf{Key Observation} &
\textbf{Design Implication} \\
\hline
\textbf{P1: End-to-end semantic security} &
System-level correctness &
Semantic correctness arises from interactions among learned and non-learned components across the entire SemCom pipeline. &
Defenses must address vulnerabilities at semantic encoders/decoders, channel effects, shared knowledge, and multi-agent coordination, rather than protecting individual models in isolation. \\
\hline
\textbf{P2: Time--location aligned defense} &
Intervention alignment &
Defenses differ in \emph{when} they act (training-time, inference-time, certified) and \emph{where} they intervene within the pipeline. &
Effective protection requires mapping defense mechanisms to concrete intervention points at the model, channel, knowledge-base, and network levels. \\
\hline
\textbf{P3: Semantically efficient robustness} &
Cost-aware robustness &
SemCom operates under strict constraints on rate, latency, energy, and computation. &
Defense mechanisms should maximize semantic fidelity or task robustness per unit cost, avoiding excessive redundancy or model complexity that negates SemCom efficiency gains. \\
\hline
\textbf{P4: Layered and composable defenses} &
Cross-layer protection &
No single defense is sufficient to secure system-level semantics in SemCom. &
Layered defenses across pipeline stages enable complementary protection, adaptive responses, and safety envelopes for critical components. \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{Layered defense taxonomy for semantic communication security based on AI defenses.}
\label{tab:defense_taxonomy}
\renewcommand{\arraystretch}{1.2}
\footnotesize
\begin{tabular}{|p{0.08\linewidth}|p{0.14\linewidth}|p{0.35\linewidth}|p{0.26\linewidth}|}
\hline
\centering\textbf{Defense Layer} & \centering\textbf{Defense Category} & \centering\textbf{Description} & \centering\arraybackslash\textbf{Methods} \\ \hline
\multirow{4}{0.08\linewidth}{\centering\textbf{Encoder/ Decoder-Level}} 
& Adversarial and \newline
Robust Training 
& Operates on semantic neighborhoods defined by meaning-preserving transformations rather than pixel- or waveform-level perturbations.
& Semantic-level adversarial training, \newline 
architectural adversarial training (e.g., masked VAE~\cite{hu2023robust}). \\ \cline{2-4}
& Representation \newline
Shaping 
& Shapes the geometry and invariances of learned semantic representations.
& Latent-space regularization, masked or quantized codebooks~\cite{hu2023robust, chen2024lightweight}, \newline complementary semantic \newline consistency~\cite{peng2022robust,peng2024robust_text}. \\ \cline{2-4}
& Generative \newline Correction and \newline Semantic Restoration 
& Corrects corrupted semantic representations at inference time by projecting noisy signals or latent codes back onto semantically plausible content. 
\newline Serves a dual role by acting as adaptive attackers during training and as semantic purifiers at inference.
& GAN~\cite{weng2024ross}, diffusion-based pre- and post-processors~\cite{weng2025generative}, generative purification~\cite{song2018pixeldefend}. \\ \cline{2-4}
& Joint Source-\newline
Channel-Security Coding 
& Neural encoders are trained so that latent representations simultaneously enable reliable semantic recovery at the intended receiver while remaining statistically uninformative to eavesdroppers.
& Deep joint source-channel and encryption coding~\cite{tung2023deepjscec}. \\ \hline
\multirow{3}{0.08\linewidth}{\centering\textbf{Channel-Level}} 
& Adversarial \newline Channel Modeling 
& Models the wireless channel as a composition of stochastic fading and physically realizable adversarial perturbations.
& Diffusion-based secure DeepJSCC\newline ~\cite{zhao2025secdiff}, task- and context-adaptive models \newline ~\cite{wijesinghe2025taco}, sparse semantic coding schemes \newline ~\cite{zhan2025sparse}. \\ \cline{2-4}
& Semantic-Aware Channel Coding 
& Allocates channel resources asymmetrically according to semantic importance.
& Deep JSCC~\cite{bourtsoulatze2019deep}, semantic importance maps~\cite{peng2024robust_image, peng2025deepscri}. \\ \cline{2-4}
& Semantic Anti-\newline Jamming and \newline Adaptive Reception 
& Targets task-level meaning rather than maximizing bit errors, allowing attacks to remain effective even when signal-level metrics appear benign.
& GAN-inspired adversarial frameworks \newline ~\cite{tang2023gan_jamming}, coding-enhanced jamming \newline schemes~\cite{chen2025coding_jamming}. \\ \hline
\multirow{3}{0.08\linewidth}{\centering\textbf{Knowledge-Base-Level}} 
& Secure Knowledge \newline Construction \newline and Maintenance 
& Ensures the ingestion, update, and evolution of semantic KBs are explicitly secured.
& Provenance-aware KB pipelines, secure maintenance workflows~\cite{yang2024secure}. \\ \cline{2-4}
& Controlled Know-\newline ledge Sharing \newline and Synchronization 
& Regulates how semantic knowledge is shared and synchronized across devices, agents, and administrative domains.
& Authenticated synchronization \newline policies~\cite{lu2024efficient, tian2025model}, knowledge management layers~\cite{liu2025knowledge, liang2024generative}. \\ \cline{2-4}
& Secure Knowledge-\newline Assisted Semantic \newline Coding 
& Integrates structured knowledge directly into semantic encoding and decoding in a security-aware manner.
& Verified knowledge sources and cross-source consistency integration~\cite{hu2022knowledge, yang2024secure, liu2024semantic}, public and private knowledge separation~\cite{liu2025knowledge}. \\ \hline
\multirow{3}{0.08\linewidth}{\centering\textbf{Network-Level}} 
& Reliability-Oriented Semantic Networking 
& Reduces semantic failure from multi-hop transmission and multi-agent propagation.
& Generative and semantic-aware correction mechanisms (e.g., InverseJSCC, GenerativeJSCC~\cite{erdemir2023generative}), diffusion models~\cite{chen2023commin}, semantic relaying~\cite{luo2022relay,ma2023intelligentrelay}. \\ \cline{2-4}
& Trust, Identity and Semantic Misbehavior Detection 
& Reasons about semantic consistency and task impact rather than packet-level authentication.
& Semantic trust establishment~\cite{gao2024esanet} and authentication mechanisms~\cite{tan2024sae}. \\ \cline{2-4}
& Feedback-Aware \newline Semantic Defense \newline Coordination 
& Feedback signals (detectors, trust scores, and semantic performance metrics) must inform routing, scheduling, model selection, or fallback strategies.
& Reinforcement learning~\cite{shokrnezhad2025arc}. \\ \hline
\end{tabular}
\end{table*}

\vspace{0.5em}
\noindent
\textbf{Distinct Constraints in SemCom.}
Before delving into these layers, it is important to highlight the unique constraints that distinguish SemCom from conventional AI systems. These constraints motivate the need for specialized defenses and shape the feasibility of intervention strategies:
\begin{itemize}
  \item \textit{Lossy transmission:} Wireless channels may irreversibly degrade encoded semantics due to noise, interference, or bandwidth limits.
  \item \textit{Shared external knowledge:} SemCom pipelines often rely on external or distributed knowledge sources that introduce synchronization and poisoning risks.
  \item \textit{Resource constraints:} Semantic inference must operate under strict latency, power, communication, and computation budgets, especially in edge or IoT settings.
  \item \textit{Semantic misalignment:} Unlike natural language processing (NLP) or computer vision (CV) systems, where errors may remain syntactic, errors in SemCom can yield meaning-preserving outputs that are functionally incorrect or unsafe.
\end{itemize}
These domain-specific constraints fundamentally limit where and how robustness mechanisms can be deployed, and necessitate tight co-design with physical and network-layer operations. 

Guided by these principles and constraints, a layered defense strategy can be organized across four critical SemCom interfaces: the semantic encoder/decoder, the wireless channel, the shared knowledge base, and the distributed network context. Each layer examines how AI defense techniques can be instantiated and composed to mitigate the threat surfaces identified in Section~\ref{sec:AI-security}.

\begin{table*}[t]
\centering
\caption{Layered defense taxonomy for semantic communication security based on AI defenses.}
\label{tab:defense_taxonomy}
\small
\begin{tabular}{|p{2.0 cm}|p{3.0cm}|p{5cm}|p{3.8cm}|}
\hline
\textbf{Defense Layer} & \textbf{Defense Category} & \textbf{Characteristics} & \textbf{Methods} \\
\hline
\multirow{4}{*}{\makecell{\textbf{Encoder/}\\\textbf{Decoder-}\\\textbf{Level}}} 
& \makecell{Adversarial \&\\ Robust Training} 
& Operates on semantic neighborhoods \\defined by meaning-preserving \\transformations rather than pixel- or \\waveform-level perturbations.
& Semantic-level adversarial training,\\ Architectural adversarial training \\(e.g., masked VAE~\cite{hu2023robust}). \\
\cline{2-4}
& \makecell{Representation\\ Shaping} 
& Shape the geometry and invariances of learned semantic representations.
& Latent-space regularization, \\Masked or quantized codebooks~\cite{hu2023robust, chen2024lightweight}, \\Complementary semantic consistency~\cite{peng2022robust,peng2024robust_text}.\\
\cline{2-4}
& \makecell{Generative\\ Correction \&\\ Semantic\\ Restoration} 
& Correct corrupted semantic representations \\at inference time by projecting noisy \\signals or latent codes back \\onto semantically plausible content. \\Serve a dual role by acting \\as adaptive attackers during \\training and as semantic purifiers \\at inference.
& GAN ~\cite{weng2024ross}, Diffusion-based pre- and post-processors ~\cite{weng2025generative}, Generative purification~\cite{song2018pixeldefend}.\\
\cline{2-4}
& \makecell{Joint Source-\\Channel-\\Security Coding} 
& Neural encoders are trained \\so that latent representations \\simultaneously enable reliable semantic \\recovery at the intended receiver \\while remaining statistically uninformative \\to eavesdroppers.
& Deep joint source--channel and encryption coding~\cite{tung2023deepjscec}.\\
\hline
\multirow{3}{*}{\makecell{\textbf{Channel-}\\\textbf{Level}}} 
& \makecell{Adversarial\\ Channel\\ Modeling} 
& Model the wireless channel as a \\composition of stochastic fading \\and physically realizable adversarial \\perturbations.
& Diffusion-based secure DeepJSCC~\cite{zhao2025secdiff}, \\task- and context-adaptive models~\cite{wijesinghe2025taco}, \\Sparse semantic coding schemes~\cite{zhan2025sparse}.\\
\cline{2-4}
& \makecell{Semantic-Aware\\ Channel Coding } 
& Allocate channel resources asymmetrically \\according to semantic importance.
& Deep JSCC~\cite{bourtsoulatze2019deep}, \\semantic importance maps~\cite{peng2024robust_image, peng2025deepscri}.\\
\cline{2-4}
& \makecell{Semantic Anti-\\Jamming \&\\ Adaptive\\ Reception} 
& Target task-level meaning \\rather than maximizing bit errors, \\allowing attacks to remain effective even when signal-level \\metrics appear benign.
& GAN-inspired adversarial frameworks\newline ~\cite{tang2023gan_jamming}\\, Coding-enhanced jamming schemes~\cite{chen2025coding_jamming}.\\
\hline
\multirow{3}{*}{\makecell{\textbf{Knowledge-}\\\textbf{Base-}\\\textbf{Level}}} 
& \makecell{Secure Knowledge\\ Construction \&\\ Maintenance} 
& Ensure the ingestion, update, \\and evolution of semantic KBs \\must be explicitly secured.
& Provenance-aware KB pipelines, \\Secure maintenance workflows~\cite{yang2024secure}.  \\
\cline{2-4}
& \makecell{Controlled\\ Knowledge\\ Sharing \&\\ Synchronization} 
& Regulate how semantic knowledge is shared and synchronized across devices, agents, and administrative domains.    
& Authenticated synchronization policies \cite{lu2024efficient, tian2025model}, Knowledge management layers ~\cite{liu2025knowledge, liang2024generative}.\\
\cline{2-4}
& \makecell{Secure Knowledge-\\Assisted Semantic\\ Coding} 
& Integrates structured knowledge directly into semantic encoding and decoding in a security-aware manner.
& Verified knowledge sources and cross-source consistency integration ~\cite{hu2022knowledge, yang2024secure, liu2024semantic},  Public and private knowledge separation ~\cite{liu2025knowledge}.\\
\hline
\end{tabular}
\end{table*}

\subsection{Encoder/Decoder-Level Defenses}\label{subsec:encdec}
Guided by the design philosophy outlined above, we begin by examining defenses at the semantic encode/decoder level. This level is the most direct interface between AI security and SemCom: it is where meaning is first abstracted into learned representations and where semantic errors most immediately translate into task failure. {As a result, many vulnerabilities and defenses studied in model-centric AI security reappear here as direct effects on semantic representations and task performance.}

Accordingly, existing encoder/decoder-level defenses in SemCom can be broadly grouped into categories that enforce robustness explicitly through adversarial optimization, implicitly through representation shaping, or structurally through generative correction and joint coding.

\begin{enumerate}
    \item \emph{Adversarial and robust training of semantic encoders and decoders.} 
This category extends adversarial training from pixel- or waveform-level perturbations to \emph{semantic neighborhoods} defined by meaning-preserving transformations. Rather than norm-bounded noise, adversaries are constructed through paraphrasing, masking, reordering, or content-preserving edits that preserve syntactic validity while inducing task-level errors, enabling encoders and decoders to be trained directly against worst-case semantic failures~\cite{hu2022robust}. Robustness can be further strengthened through architectural choices such as masked Variational Autoencoder (VAE) bottlenecks that promote discrete, semantically meaningful latent codes~\cite{hu2023robust}, as well as task-aligned objectives that enforce semantic agreement across multiple views of the same content~\cite{peng2022robust,peng2024robust_text}. At a more principled level, robustness has been formalized as a minimax semantic rate--distortion problem, where training explicitly optimizes worst-case semantic distortion rather than average-case performance~\cite{wei2025robust}. Compared with standard adversarial training targeting norm-bounded perturbations~\cite{madry2018towards}, these approaches align robustness objectives with task utility and semantic correctness.

\item \emph{Representation shaping via regularization and semantic consistency.} 
Rather than explicitly generating adversarial examples, this class improves robustness by shaping the geometry and invariances of learned semantic representations. Latent-space regularization constrains encoder sensitivity by limiting Jacobian norms, spectral radii, or latent dispersion, reducing vulnerability to small but semantically harmful perturbations under noise and interference. Masked or quantized codebooks further compress semantics into compact latent spaces, shrinking the adversary’s effective action range while improving stability and efficiency~\cite{hu2023robust,chen2024lightweight}. Complementary semantic consistency constraints encode task- or knowledge-derived invariances directly into the learning objective, encouraging paraphrases or cross-lingual variants to map to nearby representations with aligned task outputs~\cite{peng2022robust,peng2024robust_text}. These techniques parallel classical stability and Lipschitz regularization in AI security~\cite{cisse2017parseval,yoshida2017spectral}, but are adapted to semantic fidelity objectives and communication constraints, making them attractive for resource-constrained SemCom deployments.

\item \emph{Generative correction and semantic restoration.} 
Instead of hardening the encoder or decoder alone, this family introduces generative modules that actively correct corrupted semantic representations at inference time by projecting noisy signals or latent codes back onto a manifold of semantically plausible content. Generative Adversarial Networks (GAN) and diffusion-based pre- and post-processors have been proposed to filter adversarial artifacts before decoding in speech and multimodal SemCom settings~\cite{weng2024ross,weng2025generative}. Generative models can also serve a dual role by acting as adaptive attackers during training and as semantic purifiers at inference~\cite{cai2025robust}. These approaches parallel generative purification in AI defense~\cite{song2018pixeldefend}, but must remain lightweight and interruptible to respect latency, computation, and energy constraints in communication systems.

\item \emph{Joint source--channel--security coding at the encoder/decoder.} 
A distinct line of work embeds robustness and confidentiality directly into the semantic transceiver architecture. Rather than treating security as an external layer or post-hoc correction, neural encoders are trained so that latent representations simultaneously enable reliable semantic recovery at the intended receiver while remaining statistically uninformative to eavesdroppers~\cite{kalkhoran2023securedeepjscc}. Representative designs such as deep joint source--channel and encryption coding unify semantic compression, channel coding, and secrecy within a single learned mapping~\cite{tung2023deepjscec}. In contrast to adversarial training or generative purification, these approaches enforce robustness and confidentiality \emph{by construction}, making them attractive when higher-layer cryptographic support is unavailable or incompatible with semantic objectives.

    % \item \emph{Adversarial and robust training of semantic encoders and decoders.} This category extends adversarial training from pixel- or waveform-level perturbations to \emph{semantic neighborhoods} defined by meaning-preserving transformations. Semantic corruption generators based on paraphrasing, masking, and content-preserving edits can be used to construct worst-case samples within a semantic neighborhood and train encoders/decoders against them~\cite{hu2022robust}. Robustness can be further strengthened by combining adversarial training with masked Variational Autoencoder (VAE) bottlenecks that force encoders to rely on discrete, semantically meaningful codes~\cite{hu2023robust}. Task-aligned objectives that enforce semantic agreement across multiple views of the same content improve robustness under both adversarial and natural corruptions~\cite{peng2022robust,peng2024robust_text}. Robustness has also been formalized as a minimax semantic rate--distortion problem, where explicitly optimizing worst-case semantic distortion yields stronger guarantees than post-hoc fine-tuning~\cite{wei2025robust}. Compared with standard adversarial training that targets norm-bounded perturbations, these methods optimize robustness with respect to task utility rather than low-level $\ell_p$ constraints~\cite{madry2018towards}.

    % \item \emph{Generative correction and semantic restoration.} Instead of hardening the encoder or decoder alone, this family introduces generative modules that project corrupted signals or latent codes back onto a manifold of plausible semantics. GAN- and diffusion-based pre- and post-processors can filter adversarial artifacts before decoding for speech and multimodal SemCom settings~\cite{weng2024ross,weng2025generative}. A generative semantic-noise model can also be reused as both an adaptive attacker during training and as a purifier at inference time~\cite{cai2025robust}. These approaches parallel generative purification in AI defense, but must remain lightweight enough to respect latency and computational budgets in communication systems~\cite{song2018pixeldefend}.

    % \item \emph{Joint source--channel--security coding at the encoder/decoder.} A distinct line of work embeds robustness and confidentiality directly into the semantic transceiver architecture. Rather than treating security as an external layer, neural encoders can be trained so that latent representations support reliable semantic recovery at the intended receiver while remaining statistically uninformative to eavesdroppers~\cite{kalkhoran2023securedeepjscc}. Representative designs such as deep joint source--channel and encryption coding unify semantic compression, channel coding, and secrecy within a single learned mapping~\cite{tung2023deepjscec}. In contrast to adversarial training or post-hoc purification, these approaches enforce robustness and confidentiality \emph{by construction} at the encoder/decoder level, making them attractive when higher-layer cryptographic support is unavailable.
\end{enumerate}

    % \item \emph{Latent-space regularization and stability constraints.} Rather than explicitly generating adversarial examples, this category shapes the geometry of the learned semantic space to limit sensitivity to perturbations. Masked or quantized codebooks can compress semantics into compact latent spaces, reducing the adversary's effective action range~\cite{hu2023robust}. Lightweight spectral and Lipschitz-style regularization can further constrain encoder Jacobians and latent dispersion, which is particularly suitable for resource-constrained SemCom devices~\cite{chen2024lightweight}. Adaptive semantic-noise generators can complement these constraints by probing encoder vulnerabilities and driving curriculum-style robust training~\cite{cai2025robust}. These techniques parallel classical Lipschitz and stability regularization in AI security, but are tuned to semantic fidelity and rate constraints~\cite{cisse2017parseval,yoshida2017spectral}.

    % \item \emph{Constraint-aware and consistency-based representation learning.} Several works encode task- or knowledge-derived invariances directly into the learning objective. Auxiliary intent- and concept-consistency heads can encourage paraphrases, reordered descriptions, or cross-lingual variants to map to nearby latent representations and yield aligned task outputs~\cite{peng2022robust,peng2024robust_text}. Compared with purely norm-bounded robustness, such constraints exploit semantic structure that cannot be captured by simple $\ell_p$ neighborhoods. Related ideas also appear in contrastive and self-supervised learning, where positive pairs are defined by semantic relations rather than instance identity, yielding representations that are more transferable and robust to distribution shifts.
    
Overall, encoder/decoder-level defenses in SemCom closely mirror the AI security toolbox, including adversarial training~\cite{madry2018towards}, stability regularization~\cite{cisse2017parseval,yoshida2017spectral}, consistency-based learning, and generative purification~\cite{song2018pixeldefend}. However, they differ fundamentally in evaluation criteria and operating constraints. Robustness in SemCom is evaluated not by $\ell_p$ distortion or bit error rate, but by task-level semantic utility, often assessed via BLEU score~\cite{papineni2002bleu}, semantic similarity~\cite{cer2017semeval}, or downstream accuracy under rate, latency, and energy budget constraints in wireless systems.

Despite promising advances, several challenges remain. Most existing defenses assume static or bounded semantic perturbations and are developed for single-shot inference, lacking support for multi-turn or interactive SemCom workflows where feedback loops and adaptation play key roles. Furthermore, robustness is rarely co-optimized with rate–distortion and latency objectives, leaving open how much semantic robustness can be achieved without negating the efficiency gains of SemCom. %Evaluation benchmarks often rely on predefined simulations with abstracted channel models, limiting generalization to heterogeneous devices and over-the-air scenarios.
These gaps underscore the need for SemCom-native robustness evaluation protocols that integrate task utility, communication constraints, and system feedback. Progress will require tighter co-design across encoder training, JSCC architecture, and physical-layer dynamics, where robustness is not bolted on, but emerges from end-to-end semantic fidelity under adversarial and constrained conditions.


\subsection{Channel-Level Defenses under Semantic Objectives}\label{subsec:channel}
Wireless channels convey encoded semantic representations over noisy, interference-limited links, making them a primary locus where adversaries can induce semantic degradation under strict physical constraints. Unlike conventional attacks that aim to disrupt symbol recovery, semantic attackers may inject carefully crafted over-the-air perturbations that preserve syntactic reliability while inducing task-level semantic distortion, as discussed in Section~\ref{sec:2c_channelattack}. Channel-level defenses in SemCom must therefore operate within spectrum, power, and protocol constraints while explicitly optimizing semantic utility rather than bit-level fidelity.

Existing channel-level defenses for SemCom can be broadly grouped into three complementary categories.

\begin{enumerate}
    \item \emph{Adversarial channel modeling for robust SemCom.} 
    A direct defense strategy hardens semantic transceivers by explicitly modeling the wireless channel as a composition of stochastic fading and physically realizable adversarial perturbations constrained by power and bandwidth budgets. Semantic encoders and decoders are jointly trained under this mixed channel to optimize worst-case task utility rather than bit-level fidelity~\cite{nan2023physical}. Extensions of this approach incorporate diffusion-based secure DeepJSCC to improve robustness against structured adversarial interference~\cite{zhao2025secdiff}, task- and context-adaptive objectives to handle non-stationary environments~\cite{wijesinghe2025taco}, and sparse semantic coding schemes that enhance resilience under dynamic channel and task variations~\cite{zhan2025sparse}. Collectively, these methods emphasize training-time exposure to realistic worst-case channels as a foundation for semantic robustness.

    \item \emph{Semantic-aware channel coding with unequal protection.} 
    A complementary line of work focuses on allocating channel resources asymmetrically according to semantic importance, ensuring that task-critical information receives stronger protection. Deep JSCC inherently exhibits unequal error protection by prioritizing salient semantic features during end-to-end training~\cite{bourtsoulatze2019deep}. Building on this property, explicit semantic importance maps have been introduced to guide adaptive power allocation, redundancy, and diversity across semantic representations~\cite{peng2024robust_image,peng2025deepscri}. These approaches resemble cost-sensitive robust optimization in AI, but must additionally respect physical-layer constraints such as spectral efficiency, latency, and transmit power.

    \item \emph{Semantic anti-jamming and adaptive reception.} 
    Semantic jamming targets task-level meaning rather than maximizing bit errors, allowing attacks to remain effective even when signal-level metrics appear benign. Recent defenses therefore operate at the semantic level, either by co-training receivers against learned semantic jammers or by embedding coding-aware interference strategies that selectively degrade an eavesdropper while preserving legitimate semantic recovery. Representative examples include GAN-inspired adversarial frameworks that jointly train a semantic jammer and a robust receiver~\cite{tang2023gan_jamming}, as well as coding-enhanced jamming schemes that strengthen secrecy through encoder-side design under rate and reliability constraints~\cite{chen2025coding_jamming}. These approaches highlight both the effectiveness and the adaptivity of semantic jamming, underscoring the need for dynamic, task-aware reception strategies.
\end{enumerate}

Taken together, these defenses reflect three complementary design philosophies: hardening semantic transceivers through channel-realizable adversarial training, reshaping physical and link-layer resources around semantic importance, and incorporating runtime mechanisms that adapt transmission or decoding in response to semantic-aware interference. While differing in mechanism and assumptions, all three shift the protection objective from symbol fidelity to task-level semantic utility under physically realizable attacks.

From an AI defense perspective, channel-level defenses can be viewed as robustness under structured measurement noise, where adversarial perturbations are constrained by wireless physics rather than arbitrary $\ell_p$ bounds. The defining challenge in SemCom is that robustness must be engineered jointly with spectral efficiency, latency, and regulatory constraints. Defenses cannot arbitrarily increase redundancy or computation and must interoperate with standardized physical- and link-layer protocols.

Despite growing interest, channel-level defenses remain limited by simplified channel models and narrow adversary assumptions. Most evaluations rely on AWGN or single-antenna fading channels and do not capture dense, multi-user, or multi-RAT environments where attackers may exploit protocol features and scheduling dynamics. Interactions with cryptographic mechanisms such as PHY-layer authentication and link encryption are also underexplored, as semantic robustness and confidentiality are often treated as separate objectives. A key takeaway is that channel-level defenses should be evaluated using SemCom-native metrics that couple semantic utility with adversarial, spectrum- and power-constrained interference, and that robust transceiver design should be co-optimized with adaptive, attack-aware resource management.

% \begin{enumerate}
%     \item \emph{Adversarial channel modeling for robust SemCom.} A direct defense strategy is to incorporate physically realizable adversarial perturbations into the JSCC training loop by modeling the channel as a composition of stochastic fading and an adversarial transformation constrained by realistic power and bandwidth budgets. Semantic encoders and decoders are trained jointly under this mixed channel to optimize worst-case task utility rather than bit-level fidelity~\cite{nan2023physical}. Subsequent work has broadened this channel-robustness line in complementary directions, including diffusion-aided secure DeepJSCC designs against adversarial attacks~\cite{zhao2025secdiff}. Robustness under non-stationary tasks and contexts has also been explored through task adaptation and context embedding mechanisms that reshape the transceiver objective under distribution shifts~\cite{wijesinghe2025taco}. In addition, robust semantic transmission in dynamic environments has been studied via sparse vector coding structures that improve resilience to channel and semantic variations~\cite{zhan2025sparse}.

%     \item \emph{Semantic-aware channel coding with unequal protection.} A complementary line of work introduces semantic-aware unequal protection mechanisms, in which channel resources are deliberately allocated asymmetrically based on semantic importance. Deep JSCC inherently provides unequal error protection, as salient image regions are implicitly prioritized during learning~\cite{bourtsoulatze2019deep}. Building on this insight, semantic importance maps can guide adaptive power allocation, redundancy, and diversity across semantic features~\cite{peng2024robust_image,peng2025deepscri}. These approaches resemble cost-sensitive robust optimization in AI, where different features incur different robustness weights, but must additionally respect physical-layer constraints.

%     \item \emph{Semantic anti-jamming and adaptive reception.} Semantic jamming aims to corrupt or degrade semantic fidelity without triggering signal-level alarms rather than maximizing bit errors, and thus poses challenges beyond classical anti-jamming. Recent defenses therefore increasingly target \emph{task-level} degradation directly, either by co-training the receiver against learned semantic jammers or by embedding coding-aware jamming components that selectively impair an eavesdropper while preserving legitimate semantic recovery. A GAN-inspired framework trains a semantic jammer to craft over-the-air perturbations that maximize semantic mismatch and simultaneously co-trains the receiver to suppress such attacks~\cite{tang2023gan_jamming}. Complementarily, a coding-enhanced strategy injects structured interference over wiretap channels so that secrecy is strengthened through encoder-side design while maintaining the intended receiver's semantic fidelity under rate and reliability constraints~\cite{chen2025coding_jamming}. While these designs improve robustness in adversarial environments, they also illustrate how quickly a semantic jammer can adapt when it observes the same codec and task.

% \end{enumerate}

% Overall, channel-level defenses for SemCom can be summarized into three complementary families: hardening the transceiver through channel-realizable adversarial training, reshaping physical/link-layer resources around semantic importance, and incorporating runtime mechanisms that detect semantic-aware interference and adapt transmission or decoding accordingly. While these families differ in mechanism and assumptions, they share a common design principle of shifting the protection objective from bit-level fidelity to task-level semantic utility under physically realizable attacks. This shift is often operationalized through semantic-aware closed loops that monitor task-level degradation and adjust transmission or decoding policies under interference.


\subsection{Knowledge-Base-Level Defenses}\label{subsec:kb}
A distinguishing feature of SemCom systems is their reliance on shared or external semantic knowledge to guide encoding and decoding. Knowledge bases (KBs), pretrained foundation models, ontologies, and structured memories serve as semantic priors that enable aggressive compression and robust reconstruction under limited communication resources.  \emph{Despite their central role, the security implications of semantic knowledge have received comparatively limited attention relative to encoder- and channel-level defenses.}

As discussed in Section~\ref{sec:IIID_knowlegdeThreat}, this reliance introduces a unique attack surface: semantic failures may arise from manipulation, inconsistency, or overexposure of knowledge, even when learned encoders, decoders, and wireless channels behave nominally. Because semantic knowledge influences both what information is transmitted and how it is interpreted, attacks on the knowledge layer can silently induce semantic misalignment without triggering signal-level anomalies.

Existing KB-level defenses for SemCom can be broadly grouped into three complementary categories.

\begin{enumerate}
    \item \emph{Secure knowledge construction and maintenance.} 
    The first line of defense treats the semantic KB as a critical system asset whose ingestion, update, and evolution must be explicitly secured. Threats to semantic KBs have been systematized, with poisoning, tampering, and stale or inconsistent updates identified as primary risk factors~\cite{shen2023secure}. Provenance-aware KB pipelines tag each update with source identity, temporal metadata, and verification status, enabling suspicious or conflicting updates to be quarantined or rolled back. Secure maintenance workflows can further incorporate access control, logging, and auditability to bound the blast radius of compromised contributors and support post-hoc forensic analysis~\cite{yang2024secure}. These mechanisms parallel data lineage and governance practices in secure ML pipelines, but are uniquely critical in SemCom because KB corruption affects both semantic compression and reconstruction.

    \item \emph{Controlled knowledge sharing and synchronization.} 
    The second category focuses on regulating how semantic knowledge is shared and synchronized across devices, agents, and administrative domains. SemCom systems often implicitly assume sufficiently aligned knowledge at the transmitter and receiver; adversaries can exploit partial synchronization, delayed updates, or version mismatches to induce semantic divergence without disrupting signal delivery. Recent works therefore distinguish between global knowledge and private or personalized knowledge, and enforce authenticated synchronization policies \cite{lu2024efficient,tian2025model}. A dedicated knowledge management layer can coordinate access control, update authentication, and selective synchronization, preventing adversaries from reconstructing the exact semantic context used by legitimate endpoints~\cite{liu2025knowledge}. From a defense standpoint, such mechanisms act as semantic access control, limiting both semantic leakage and desynchronization-induced misinterpretation.

    \item \emph{Secure knowledge-assisted SemCom pipeline.} 
    Rather than treating knowledge solely as a background resource, this category integrates structured knowledge directly into semantic encoding and decoding in a security-aware manner. Knowledge-assisted semantic coding schemes inject graph-based or symbolic priors into representation learning so that encoders compress messages in ways consistent with trusted knowledge, while decoders use knowledge-guided reasoning to recover missing semantics under noise. Incorporating verified knowledge sources and cross-source consistency checks can improve robustness against both channel noise and semantic ambiguity~\cite{hu2022knowledge,yang2024secure,liu2024semantic}. More recent designs emphasize separating public and private knowledge during encoding, such that accurate semantic reconstruction requires access to the intended private knowledge context~\cite{liu2025knowledge}. This effectively turns private knowledge into an implicit security key: even if an adversary intercepts semantic representations and possesses strong global priors, the absence of synchronized private knowledge prevents correct interpretation of sensitive semantics.
\end{enumerate}

From an AI defense viewpoint, KB-level defenses share commonalities with robust data management, trustworthy knowledge graphs, and secure retrieval-augmented generation. Provenance tracking and access control mirror secure data pipelines in ML, while robust graph learning limits the influence of corrupted nodes or edges during message passing. The key distinction in SemCom is that KB integrity and availability directly influence \emph{both} encoding and decoding behavior. Small perturbations in knowledge can therefore induce large semantic shifts without triggering any signal-level anomaly.

Despite growing recognition of their importance, KB-level defenses remain relatively underdeveloped in SemCom. There is no standardized benchmark for evaluating robustness or privacy of semantic knowledge bases under dynamic updates and partial trust assumptions. Many proposed defenses rely on strong provenance or trust signals that may be unavailable in open or cross-domain deployments. Moreover, restricting knowledge access to improve security can complicate verification, auditing, and synchronization, creating new trade-offs between robustness, privacy, and system usability.

A key takeaway is that semantic knowledge should be treated as a first-class security asset rather than a benign background resource. Its construction, synchronization, exposure, and integration into semantic models should be co-designed with explicit robustness and privacy objectives, and evaluated under adversarial conditions that reflect realistic SemCom deployments.

% \begin{enumerate}
%     \item \emph{Secure knowledge construction and maintenance.} The first line of defense treats the semantic knowledge base as a critical system asset whose ingestion, update, and evolution must be explicitly secured. Threats to semantic knowledge bases have been systematized, with poisoning, tampering, and stale or inconsistent updates identified as primary risk factors~\cite{shen2023secure}. Provenance-aware KB pipelines further tag each update with source identity, temporal metadata, and verification status, enabling suspicious or conflicting updates to be quarantined or rolled back~\cite{shen2023secure}. Secure KB maintenance workflows can additionally incorporate access control, logging, and auditability to bound the blast radius of compromised contributors and support post-hoc forensic analysis~\cite{yang2024secure}. These mechanisms parallel data lineage and governance practices in secure ML pipelines, but are uniquely critical in SemCom because KB corruption affects both semantic compression and reconstruction.

%     \item \emph{Controlled knowledge sharing and synchronization.} A second category focuses on regulating how semantic knowledge is shared and synchronized across devices, agents, and administrative domains. SemCom often implicitly assumes sufficiently aligned knowledge at the transmitter and receiver; adversaries can exploit partial synchronization, delayed updates, or version mismatches to induce semantic divergence. Recent works therefore distinguish between global knowledge and private or personalized knowledge and enforce authenticated synchronization policies. A knowledge management layer can coordinate access control, update authentication, and selective synchronization, preventing adversaries from reconstructing the exact semantic context used by legitimate endpoints~\cite{liu2025knowledge}. From a defense standpoint, such mechanisms act as semantic access control, limiting both semantic leakage and desynchronization-induced misinterpretation.
    
%     \item \emph{Knowledge exploitation in SemCom pipeline.} Rather than treating knowledge solely as a background resource, several works integrate structured knowledge directly into semantic encoding and decoding in a security-aware manner. Knowledge-assisted semantic coding schemes inject graph-based or symbolic priors into representation learning so that encoders compress messages in ways consistent with trusted knowledge, while decoders use knowledge-guided reasoning to recover missing semantics under noise. Incorporating verified knowledge sources and cross-source consistency checks can improve robustness against both channel noise and semantic ambiguity~\cite{hu2022knowledge,yang2024secure}. More recent designs emphasize separating public and private knowledge during encoding, such that accurate semantic reconstruction requires access to the intended private knowledge context~\cite{liu2025knowledge}. This effectively turns private knowledge into an implicit security key: even if an adversary intercepts semantic representations and possesses strong global priors, the absence of synchronized private knowledge prevents correct interpretation of sensitive semantics.
% \end{enumerate}

% From an AI defense viewpoint, KB-level defenses share commonalities with robust data management, trustworthy knowledge graphs, and secure retrieval-augmented generation. Provenance tracking and access control mirror secure data pipelines in ML, while robust graph learning limits the influence of corrupted nodes or edges during message passing. The key distinction in SemCom is that KB integrity and availability directly influence \emph{both} encoding and decoding behavior. Small perturbations in knowledge can therefore induce large semantic shifts without triggering any signal-level anomaly.

% Despite growing recognition of their importance, KB-level defenses remain relatively underdeveloped in SemCom. There is no standardized benchmark for evaluating robustness or privacy of semantic knowledge bases under dynamic updates and partial trust assumptions. Many proposed defenses rely on strong provenance or trust signals that may be unavailable in open or cross-domain deployments. Moreover, restricting knowledge access to improve security can complicate verification, auditing, and synchronization, creating new trade-offs between robustness, privacy, and system usability.

% A key takeaway is that semantic knowledge should be treated as a first-class security asset rather than a benign background resource. Its construction, synchronization, exposure, and integration into semantic models should be co-designed with explicit robustness and privacy objectives, and evaluated under adversarial conditions that reflect realistic SemCom deployments.


\subsection{Network-Level Defenses}\label{subsec:network}
Unlike encoder-, channel-, or knowledge-level defenses, network-level defenses address semantic failures that emerge from interaction, propagation, and coordination among multiple terminals over time, rather than from any single compromised component. In networked SemCom systems, meaning is not only decoded locally but also propagated, aggregated, and acted upon across agents, making semantic security an inherently collective property.

From an AI defense perspective, network-level semantic defenses parallel robust multi-agent learning, distributed anomaly detection, and trust-aware decision-making under adversarial conditions. Generative correction mechanisms resemble robust generative modeling under distribution shift, while trust evaluation and authentication mirror reputation systems in adversarial multi-agent environments. The key distinction in SemCom is that the protected object is not packet delivery or throughput, but the consistency and integrity of shared meaning as it propagates through the network.

Existing network-level defenses for SemCom can be broadly grouped into three categories.

% Unlike encoder-, channel-, or knowledge-level defenses, network-level defenses address semantic failures that emerge from interaction, propagation, and coordination among multiple terminals, rather than from any single compromised component.  From an AI defense perspective, network-level semantic defenses closely parallel robust multi-agent learning, distributed anomaly detection, and trust-aware decision-making under adversarial conditions. Generative correction mechanisms resemble robust generative modeling under distribution shift, while trust evaluation and authentication mirror reputation systems and behavior modeling in adversarial multi-agent environments. The key distinction in SemCom is that the protected object is not packet delivery or throughput, but the consistency and integrity of shared meaning as it propagates across the network.


\begin{enumerate}
    \item \emph{Reliability-oriented semantic networking and cooperative robustness.} 
    The first category addresses semantic failures that emerge from multi-hop transmission and multi-agent propagation, where small local distortions can accumulate into global task failure. Generative and semantic-aware correction mechanisms can be deployed at intermediate nodes, relays, or edge servers to stabilize semantics before forwarding. Representative examples include InverseJSCC and GenerativeJSCC, which use generative models to denoise or reconstruct semantically plausible outputs from heavily corrupted DeepJSCC transmissions~\cite{erdemir2023generative}. Semantic reconstruction has also been formulated as an inverse problem, combining invertible neural networks with diffusion models to recover high-quality semantics from degraded intermediate representations~\cite{chen2023commin}. 
    Beyond pure correction, intelligent semantic relaying allows intermediate nodes to partially decode, refine, or re-encode semantic information using shared or local knowledge, reducing semantic drift across hops~\cite{luo2022relay,ma2023intelligentrelay}. Collectively, these approaches act as network-level semantic filters that prevent localized corruption from cascading through the system.

    \item \emph{Trust, identity, and semantic misbehavior detection.} 
    Even when links are reliable, adversaries may impersonate legitimate agents, inject malicious semantic content, or manipulate coordination protocols. Network-level defenses therefore extend beyond packet-level authentication to reasoning about semantic consistency and task impact. Trust establishment and authentication can leverage semantic and environmental features that are difficult to forge at scale, such as environment-level semantics extracted from massive MIMO channels for physical-layer authentication~\cite{gao2024esanet}. Authentication mechanisms have also been co-designed with semantic objectives through metrics that explicitly balance authentication reliability and throughput~\cite{tan2024sae}. 
    More broadly, misbehavior detection in SemCom networks must identify agents whose semantic outputs systematically distort shared meaning or degrade task performance, even when syntactic validity is preserved.

    \item \emph{Feedback-aware semantic defense coordination.} 
    A third category treats semantic defense as a coordinated, adaptive process across the network rather than a static mechanism at individual nodes. In this view, detectors, trust scores, and semantic performance metrics serve as feedback signals that inform routing, scheduling, model selection, or fallback strategies. Detection of semantic jamming or anomalous behavior at one node can trigger route changes, decoder switching, or semantic rate adaptation elsewhere in the network~\cite{gao2025agenticsemcom}. Although still in an early stage, such orchestration aligns closely with AI-based control and reinforcement learning frameworks for autonomous networks~\cite{shokrnezhad2025arc}. 
    From an AI defense perspective, these mechanisms resemble robust multi-agent learning and trust-aware decision-making, with the key distinction that SemCom networks protect \emph{shared meaning and semantic coherence}, rather than packet delivery or throughput alone.
\end{enumerate}

Despite their importance, network-level defenses for SemCom remain limited. Many existing schemes assume benign cooperation or random impairments and do not explicitly model adaptive adversaries that exploit network dynamics, feedback loops, or generative priors. Scalability and latency pose additional challenges: trust management and generative correction may introduce communication, computation, and coordination overhead that is incompatible with real-time semantic tasks. Moreover, trust is often defined at the agent level rather than at the level of semantic content or knowledge items, leaving open how to quantify, propagate, and act on trust in meaning itself.

A key takeaway is that semantic security is an emergent, system-level property. Ensuring robustness in networked SemCom requires defenses that jointly reason over agents, links, knowledge, and tasks, and that enable graceful degradation under partial compromise rather than catastrophic failure.

% \begin{enumerate}
%     \item \emph{Reliability-oriented semantic networking and cooperative robustness.} A first line of defense mitigates the accumulation and propagation of semantic distortion across multiple hops or agents. Generative and semantic-aware correction mechanisms can be deployed at intermediate nodes, relays, or edge servers to restore or stabilize semantics before forwarding. InverseJSCC and GenerativeJSCC use generative models to denoise or reconstruct semantically plausible outputs from heavily corrupted DeepJSCC transmissions~\cite{erdemir2023generative}. Semantic reconstruction has also been formulated as an inverse problem, combining invertible neural networks with diffusion models to recover high-quality semantics from degraded intermediate representations~\cite{chen2023commin}. Intelligent semantic relaying can further improve robustness by allowing relays to partially decode, refine, or re-encode semantic information using shared or local knowledge, reducing semantic drift across hops~\cite{luo2022relay,ma2023intelligentrelay}. These approaches can be viewed as network-level semantic filters that prevent local corruption from cascading into global task failure.
    
%     \item \emph{Trust, identity, and misbehavior detection in semantic networks.} Even when links are reliable, adversaries may impersonate legitimate agents, inject malicious semantic content, or manipulate coordination protocols. Trust establishment and authentication can leverage semantic and environmental features that are difficult to forge at scale. Environment-level semantics extracted from massive MIMO channels have been used as robust fingerprints for physical-layer authentication~\cite{gao2024esanet}. Authentication mechanisms have also been co-designed with semantic objectives via metrics that explicitly balance authentication reliability and throughput~\cite{tan2024sae}. More broadly, misbehavior detection in SemCom networks must reason about \emph{semantic consistency} and \emph{task impact}, rather than only packet anomalies, to reliably identify malicious agents and poisoned messages.
    
%     \item \emph{Feedback-aware semantic defense coordination.} A third category treats defense as a coordinated, adaptive process across the network rather than a static mechanism at individual nodes. In this view, detectors, trust scores, and semantic performance metrics serve as feedback signals that inform routing, scheduling, model selection, or fallback strategies, such that detection of semantic jamming or anomalous behavior at one node can trigger route changes, model switching, or semantic rate adaptation elsewhere in the network~\cite{gao2025agenticsemcom}. Although still in an early stage, such orchestration aligns closely with AI-based control and reinforcement learning frameworks used in autonomous networks~\cite{shokrnezhad2025arc}. From an AI defense standpoint, network-level defenses resemble robust multi-agent learning, distributed anomaly detection, and trust-aware decision-making, where generative correction parallels robust generative modeling under distribution shift and trust evaluation mirrors reputation systems and behavior modeling in adversarial multi-agent environments. The key distinction in SemCom is that the objects being protected are \emph{semantic representations and shared meaning}, not merely packet delivery or throughput.

% \end{enumerate}

% In general, many existing schemes assume benign cooperation or random impairments and do not explicitly model adaptive adversaries that exploit network dynamics, feedback loops, or generative priors. Scalability and latency remain major constraints: trust management and generative correction can introduce communication, computation, and coordination overhead that is incompatible with real-time semantic tasks. Moreover, trust is often defined at the agent level rather than at the level of semantic content or knowledge items, leaving open how to quantify, propagate, and act on trust in meaning itself.

% A key takeaway is that semantic security is an emergent, system-level property. Ensuring robustness in networked SemCom requires defenses that reason jointly over agents, links, knowledge, and tasks, and that enable graceful degradation under partial compromise rather than catastrophic failure.


% \subsection{Cross-Domain Lessons and Integration Paths}
% Defensive strategies in SemCom, particularly at the encoder and decoder levels, naturally intersect with robustness techniques developed in natural language processing (NLP) and computer vision (CV). These mature fields offer valuable design insights and benchmarking practices, given that all three domains rely on learned representations that encode semantic meaning and must resist adversarial perturbations.

\subsection{Cross-Domain Lessons and Integration Paths}
The layered defenses discussed above demonstrate that securing SemCom requires coordinated protection across representation learning, physical transmission, shared knowledge, and networked interaction. At each layer, many proposed mechanisms draw inspiration implicitly or explicitly from robustness techniques developed in mature AI domains, particularly NLP and CV. To place these defenses in a broader context and to identify paths toward principled integration, it is instructive to examine how related challenges have been addressed in NLP and CV.

Both NLP and CV confront adversaries that manipulate learned representations to alter meaning without obvious syntactic corruption, a threat model that closely mirrors semantic attacks in SemCom. However, while robustness techniques in these domains are typically developed for standalone inference pipelines, SemCom embeds learned models within communication-constrained, distributed systems where robustness must coexist with rate, latency, energy, and coordination constraints. This subsection distills transferable lessons from NLP and CV robustness, clarifies where direct adoption breaks down, and outlines integration paths for developing SemCom-native defenses that respect system-level constraints.

\paragraph{Transferable Ideas from NLP and CV Robustness}
In NLP, consistency-based learning and semantic-preserving perturbations, such as paraphrasing or synonym substitution, have improved robustness against ambiguity and adversarial rewriting~\cite{wang2022measure,goyal2023survey}. Similarly, in CV, defenses have evolved from norm-bounded perturbation resistance to include semantic shifts and natural distributional corruptions. Notable techniques include representation smoothing, input transformations, and ensemble-based strategies~\cite{drenkow2021systematic,li2023trade}. These advances have inspired emerging SemCom defenses, such as semantic consistency objectives~\cite{peng2022robust}, latent-space regularization~\cite{chen2024lightweight}, and generative purification~\cite{weng2025generative}, which aim to align encoded representations with underlying meaning under constrained conditions.

\paragraph{Adaptation Challenges Under SemCom Constraints}
Despite these parallels, SemCom introduces domain-specific challenges that limit direct transfer. As highlighted in the “Distinct Constraints” of Section \ref{sec:principle}, SemCom pipelines must meet strict rate, power, and latency budgets, operate over noisy and lossy physical channels, and maintain coherence with shared or external knowledge modules. Defenses must therefore be communication-aware and lightweight, often requiring co-design with encoder–decoder architectures or joint source–channel coding schemes. Standard robustness techniques from NLP or CV, such as computationally expensive adversarial training or always-on ensembles, cannot be directly applied without violating these deployment constraints.

Evaluation practices from NLP and CV also offer useful reference points. Benchmark datasets like ImageNet-C~\cite{hendrycks2019benchmarking} and adversarial GLUE~\cite{nie2020adversarial} have catalyzed standardized robustness evaluation. A SemCom analog should incorporate over-the-air channel traces, semantic misalignment detection, and knowledge desynchronization scenarios that reflect practical operation. These additions would encourage evaluation under constraints that match the semantic and physical realities of deployment.

\paragraph{Integration Paths for SemCom-Native Robustness}
To meaningfully integrate these lessons, robustness in SemCom should be treated as a system-level resource allocation problem. Rather than uniformly deploying defenses, protection budgets, such as redundancy, abstention, or adaptive filtering, should be allocated based on marginal utility under task priorities and system constraints. Lightweight mechanisms such as real-time anomaly detection, fallback control strategies, or contract-based semantic monitoring may offer better tradeoffs than heavy, static defenses.

Future SemCom pipelines will benefit from semantically aware, composable defenses that are compatible with constrained environments and adversarial uncertainty. These defenses should be designed with explicit assumptions, verified through contextual testing, and reported using deployment-aware robustness profiles rather than isolated metrics. Lessons from NLP and CV robustness will be instrumental in shaping these systems, but success will require adapting them to the unique architectural and operational demands of SemCom.

==> 6_backup.tex <==
\section{Bridging Design and Deployment for Secure Semantic Communications} \label{sec:deployment}

\begin{figure*}[!t]
\centering
\includegraphics[width=1.0\textwidth]{figures/section5.pdf}
\caption{Bridging design and deployment through operating envelopes and runtime control in secure semantic communication. Robustness is enforced as a managed system property via a semantic control plane that integrates operating-envelope awareness, resource and priority telemetry, policy coordination, and cross-layer consistency signals from the AI-defense lens.}
\label{fig:sec5}
\end{figure*}


Despite advances in semantic encoding, adversarial robustness, and threat detection, many SemCom defenses have not yet adopted them in practical systems. To bridge the gap between principled designs and practical systems, it requires system architectures capable of runtime introspection, policy enforcement, and adaptive behavior under stringent resource constraints. This section discusses three major difficulties of deploying secure SemCom based on AI security: managing security–utility tradeoffs within constrained operating envelopes, enforcing robustness without violating resource or timing constraints, and supporting verifiable behavior through semantic-level certification. %These challenges converge in (D), which addresses composed failure modes—emergent system breakdowns caused by cross-layer misalignments even when individual modules perform as intended.

\subsection{Security–Utility Tradeoffs and Operating Envelopes}
Security mechanisms applied in SemCom often conflict with task utility, latency, and energy constraints. While these defenses improve robustness under attack or drift, they impose computational or communication overhead that can degrade system throughput or violate timing budgets. This creates a core tension: securing SemCom systems cannot be done in isolation from their performance envelopes.

To reason about these tradeoffs, we adopt the notion of \textit{operating envelopes}: regions in the multidimensional space of semantic utility, latency, robustness, and system cost, which represent acceptable operating points under bounded resources and threat models. This concept, widely used in real-time and networked systems \cite{aastrom2021feedback,liu2000real}, has recently found traction in robust AI and adaptive communication design, where runtime decisions are governed by control policies operating within certified performance regions \cite{madry2018towards,zappone2019model}. Within this framework, robustness mechanisms are viewed as policy choices constrained by explicit system budgets. For instance, increasing abstention thresholds may improve resilience to semantic drift, but at the cost of higher decision latency or degraded task completion rates.

In practice, most current SemCom pipelines are tuned offline using fixed thresholds and evaluated under average-case conditions. Runtime enforcement of semantic risk budgets is largely absent. Moreover, the lack of standard metrics for semantic degradation under resource constraints makes it difficult to compare or certify defenses across systems. In addition, we also need to consider the resource limitations of SemCom systems. Thus, to transition from design to deployment, future SemCom systems should support \textbf{envelope-aware introspection}: mechanisms that continuously monitor semantic fidelity, latency, energy usage, and channel state to enable dynamic adjustment of semantic security policies under resource limitations. This requires not only robust semantic encoders but also coordination with lower-layer scheduling and system monitors to evaluate whether defenses remain within operating budgets.

%In the absence of such support, systems are prone to silent performance degradation or brittle failure modes when confronted with adversarial inputs, unexpected context shifts, or environmental resource constraints. Operating envelopes must become first-class objects—measurable, enforceable, and auditable across the SemCom stack.


%%\subsection{Deployment Under Resource and Priority Constraints}
%%SemCom systems are frequently deployed under strict real-time and resource constraints, where latency, energy, and compute budgets are as critical as semantic accuracy and robustness.  In practice, systems must also satisfy broader operational priorities and quality-of-service (QoS) requirements, such as reliability targets, throughput guarantees, jitter bounds, and service differentiation across traffic classes. In these settings, even modest defensive overhead such as additional detection passes, model switching, or redundancy can violate priority objectives, degrade semantic performance, or cause task failure. Thus, the core deployment challenge is not average-case robustness, but ensuring semantic integrity under worst-case resource contention and priority-driven QoS constraints.

%%Security mechanisms often interact with system constraints in unpredictable ways. Detection and purification costs may scale with channel conditions or adversarial activity. Generative correction and ensemble decoding introduce partially interruptible pipelines, while shared accelerators exacerbate contention between traffic flows. Without coordination, these layers can cause backpressure, propagate delays, or oscillate between over- and under-protection, ultimately destabilizing the system and breaking QoS guarantees.

%%To mitigate these issues, we advocate \textbf{a priority-aware defense} policy: defensive actions are admitted only when they preserve the system’s current QoS and priority objectives for the active traffic class. When resources are tight, the system should degrade gracefully under an explicit policy, for example, by using compressed semantic codes, invoking early exits, lowering decoding complexity, or reusing cached inferences. Safety- or mission-critical traffic should be assigned priority lanes with reserved compute and airtime to prevent starvation or QoS regression induced by best-effort robustness actions.

%%Robust deployment further requires tight integration across scheduling, telemetry, and semantic policy. Per-flow budgets for compute, memory, and airtime should be enforced via lightweight runtime governors. Telemetry should emphasize tail behavior (e.g., p95, p99 latency and miss rates), rather than averages. Semantic priors and channel features should be cached where feasible to reduce cold-start costs, and updates to models or knowledge bases should use non-blocking rollout strategies to maintain service continuity and avoid QoS disruptions.

%%Evaluation frameworks must reflect deployment realism by explicitly quantifying robustness under priority-relevant stressors, including bursty loads, time-varying channels, partial contention, and mixed-criticality traffic. Systems should report robustness–QoS tradeoffs, particularly for defensive paths that risk tail-latency spikes or jitter amplification. These principles are not tied to a fixed architecture but serve as general guidelines for aligning robustness mechanisms with priority-driven system constraints.

%%Ultimately, deploying semantic security under real-world constraints requires treating robustness as a resource- and policy-governed service, not a standalone capability. Priority-aware design, QoS-compliant adaptation, and tail-resilient integration are essential for operational robustness.

\subsection{Certification and Verifiable Robustness}
Certification represents a critical bridge between principled robustness analysis and deployable SemCom systems. In the SemCom context, certification is not merely about proving worst-case guarantees for isolated models, but about enabling system-level assurances that support safe and predictable behavior under real-world uncertainty. This includes certifying task-level properties, such as intent preservation or safe control actions, under physically realizable perturbations and dynamic operating conditions.

Unlike conventional AI settings, SemCom systems operate under stochastic fading, time-varying bandwidth, feedback-driven protocols, and adaptive control mechanisms. As a result, robustness guarantees are inherently multi-layered and context-dependent. While techniques such as randomized smoothing, Lipschitz bounding, and convex relaxations provide useful foundations in static learning pipelines \cite{li2023sok,zhang2022rethinking,cohen2019certified}, their assumptions rarely hold end-to-end in wireless systems. Over-the-air attackers are constrained by physical limits such as transmit power, spectral locality, and temporal coherence rather than abstract $\ell_p$ norms, and semantic utility itself may depend on protocol state, decoding slack, or application feedback. Adaptive behaviors such as HARQ, link adaptation, and semantic fallback further complicate static certification.

To address these challenges, certification in SemCom should be treated as a \emph{runtime system artifact} rather than an offline proof obligation. Certificates, such as confidence radii, abstention indicators, or semantic bounds, should be attached to semantic outputs as lightweight metadata. These signals enable downstream policy decisions, allowing defensive actions, semantic retransmissions, or safety-critical actuation to be gated based on certified guarantees, available system slack, and contextual risk.

Deployable certification further requires threat models aligned with physical-layer realities. Certifiable perturbation sets should be defined in terms of SNR ranges, error vector magnitude (EVM) bounds, or semantic edit distances that reflect realistic wireless degradation. Certification efforts should prioritize semantically stable representations, such as latent embeddings or task-specific logits, where guarantees are more meaningful and resilient to transmission variability.

Rather than producing static worst-case bounds, certified robustness should be embedded within the \emph{operating envelope} of the system. Representing certified guarantees as regions over semantic utility, latency, and power budgets enables practical reasoning about when guarantees hold and how they interact with runtime constraints. Future research directions include composing certificates across encoder–channel–decoder pipelines, caching and reusing certified inference regions, and integrating certification signals into adaptive abstention or fallback policies. Ultimately, certification in SemCom must evolve into a dynamic, observable, and composable mechanism that supports system-level decision making under real-world conditions.

%\subsection{Cross-Layer Failure and Composable Robustness}
%A fundamental challenge in secure SemCom is that robustness guarantees rarely compose across system layers. Semantic failures in deployed systems often arise not from a single broken component, but from the interaction of multiple, individually admissible perturbations across the encoder, channel, knowledge, and coordination layers. While Sections~\ref{sec:AI-security} and~\ref{sec:4layered_defense} analyzed threats and defenses at individual interfaces, real-world adversaries are not confined to a single layer. Small, coordinated manipulations applied across layers can combine to produce significant semantic degradation, even when each component operates within its assumed threat model.

%These failures are typically caused by mismatched assumptions rather than flawed mechanisms. Encoder-level defenses often assume stable channels and synchronized context. Channel-level defenses treat semantic decoders as fixed functions. Knowledge and network defenses reason about trust and integrity independently of signal-level uncertainty. When deployed together, these assumptions need not hold simultaneously. As a result, perturbations can propagate and interact in ways that were never exercised during component-level training or validation.

%This gap reflects a deeper limitation in how robustness is currently reasoned about. Most guarantees are established under single-layer perturbations and static contexts, implicitly assuming independence across layers. In practice, adversarial training, channel hardening, and trust mechanisms may interfere or amplify one another when composed, leading to brittle behavior that is difficult to diagnose post hoc. End-to-end semantic security therefore cannot be inferred from the robustness of isolated components.

%Mitigating composed failures requires system-level controls rather than further specialization at individual layers. One pragmatic approach is to evaluate robustness against \emph{joint perturbation budgets}, even if coarsely specified, to expose interaction effects early in the design process. Another is to monitor semantic consistency across layers by comparing signals such as encoder confidence, channel-induced uncertainty, and knowledge plausibility, using disagreement as a trigger for conservative system policies. These mechanisms aim to prevent silent semantic failure without requiring precise attack attribution.

%Equally important is policy-level coordination. Robustness estimates, detectors, and trust signals should feed into a unified control policy governing semantic rate, redundancy, model selection, or abstention. Treating these signals independently risks underreaction to composed threats or overreaction to benign noise. Framing defense as a control problem aligns naturally with the operating-envelope perspective introduced earlier in this section.

%Addressing cross-layer and composed failures remains a structural challenge, rooted in the absence of established methodologies for specifying joint threat models and reasoning about how local guarantees interact under adaptation and feedback. Overcoming this limitation is essential for transitioning from component-wise robustness to deployable, end-to-end semantic security. Future SemCom architectures may therefore incorporate lightweight orchestration layers, such as semantic control planes, that monitor telemetry, enforce per-flow budgets, and coordinate robustness mechanisms based on semantic divergence and system slack. In this view, cross-layer robustness becomes a managed system service: observable, auditable, and adaptive to evolving environments and adversarial conditions.

% \subsection{Certification and Verifiable Robustness in Semantic Communications}

% Certification aims to bridge formal guarantees from machine learning with the real-world variability of wireless environments. For SemCom systems, this entails certifying task-level correctness, for instance, ensuring intent preservation or verifying safe control actions, even in the presence of physically realizable perturbations. Unlike conventional AI settings, semantic communications must contend with stochastic fading, time-varying bandwidth, and feedback protocols, which make robustness guarantees inherently multi-layered and context-dependent.

% While techniques such as randomized smoothing, Lipschitz bounding, and convex relaxations have enabled formal guarantees in AI pipelines \cite{cohen2019rs,li2023sok,zhang2022rethinking}, their assumptions rarely hold in wireless settings. Over-the-air attackers are constrained not by $\ell_p$-norms, but by physical limits such as transmit power, spectral locality, and temporal constraints. Semantic utility itself may be non-smooth, coupled to protocol state, or dependent on dynamic context (e.g., decoding slack or application-level feedback). Adaptive behaviors like HARQ, link adaptation, or semantic fallback mechanisms \cite{jiang2022deep,zhou2022adaptive} further violate static modeling assumptions. As a result, robustness certificates derived from isolated components often fail to hold end-to-end.

% A more pragmatic perspective treats certification not as an offline guarantee, but as a runtime artifact embedded in the system. Certificates, such as confidence radii, abstention flags, or semantic bounds, should be attached to each output as lightweight metadata, enabling policy-based decisions downstream. These tags support runtime tradeoffs: defensive behaviors, semantic retransmissions, or safety-critical actuation can be gated based on certified guarantees, available system slack, or contextual risk estimates.

% Deployable certification further requires threat models that align with physical-layer realities. Certifiable perturbation sets should be defined using SNR bins, error vector magnitude (EVM) bounds, or semantic edit distances that reflect actual wireless degradation. Preprocessing steps, such as band-limiting or frequency masking, should be designed to match real-world attack capabilities and reduce overfitting to abstract threat models. Certification efforts should also target semantically stable representations, such as latent embeddings or task-specific logits, where guarantees are more meaningful, generalizable, and robust to transmission variations.

% To make these guarantees actionable, certified robustness should be reported as part of an \emph{operating envelope}: a compact, multi-dimensional characterization of semantic utility across SNR, latency, and power budgets. Such envelopes offer a more transparent view of system performance under uncertainty compared to static, worst-case bounds. Future directions include certificate composition across encoder-channel-decoder pipelines, runtime caching and reuse of certified inference regions, and adaptive abstention or fallback policies as safety-aware responses.

% Ultimately, certification in SemCom must evolve beyond static mathematical proofs into dynamic, system-aware mechanisms. These mechanisms should be observable, auditable, and composable, supporting robust decision-making in real-world conditions and enabling a foundation for trustworthy semantic communication.

% \subsection{Cross-Layer Failure and Composable Robustness}
% A central limitation of existing defenses is that semantic failures often arise from the \emph{composition} of otherwise admissible perturbations across multiple system components. While Sections~\ref{sec:AI-security} and~\ref{sec:semcom-defenses} analyzed threats and defenses at individual layers, practical adversaries are not confined to a single interface. Small manipulations applied jointly at the source, channel, knowledge, or coordination layers can combine to produce large semantic degradation, even when each layer operates within its assumed threat model. As a result, end-to-end semantic security cannot be inferred from the robustness of isolated components.

% These cross-layer failures are typically caused by mismatched assumptions rather than by broken mechanisms. Encoder-level defenses often assume fixed channels and synchronized context. Channel-level defenses treat semantic decoders as stable functions. Knowledge and network defenses reason about integrity and trust independently of signal-level uncertainty. When deployed together, these assumptions need not hold simultaneously, allowing perturbations to propagate and interact in ways that were not exercised during training or evaluation. This subsection does not argue for a new class of defenses. Instead, it highlights a gap between how defenses are \emph{validated} and how systems \emph{fail}. Most robustness guarantees do not compose: adversarial training, channel hardening, and trust mechanisms are typically evaluated under single-layer perturbations and static contexts. When combined, their guarantees may weaken or even interfere, producing brittle behavior that is difficult to diagnose post hoc.

% From an engineering standpoint, mitigating composed attacks requires system-level controls rather than deeper specialization at individual layers. One practical step is to evaluate robustness against \emph{joint perturbation budgets}, even if coarsely defined, to expose interaction effects early. Another is to monitor semantic consistency across layers by comparing multiple signals, such as encoder confidence, channel-induced uncertainty, and knowledge plausibility, and using disagreement as a trigger for conservative system policies. These mechanisms do not require precise attack attribution; they aim only to prevent silent semantic failure.

% Equally important is policy-level coordination. Detectors, robustness estimates, and trust signals should feed into a unified control policy governing semantic rate, redundancy, model selection, or abstention. Treating these signals independently risks underreaction to composed threats or overreaction to benign noise. Viewing defense as a control problem aligns naturally with the operating-envelope perspective introduced earlier in this section.

% Defending against cross-layer and composed attacks remains a \emph{structural challenge}, rooted in the absence of established methodologies for specifying joint threat models and for reasoning about how local guarantees interact under adaptation and feedback. Addressing this challenge is essential for moving from component-wise robustness to deployable, end-to-end semantic security.

% To support this transition, future SemCom architectures may incorporate lightweight orchestration layers—such as semantic control planes—that monitor telemetry, enforce per-flow budgets, and coordinate robustness mechanisms based on semantic divergence and system slack. These systems must remain modular and composable, allowing applications to customize semantic policies while preserving core system-level safeguards. Importantly, \textit{cross-layer robustness should be treated as a managed system service}, which is observable, auditable, and adaptive to changing environments and adversarial conditions.


% Security mechanisms in SemCom systems are tightly coupled with task utility, latency, rate, and energy. Stronger detection thresholds increase false positives and suppress useful semantic content; abstention and re-requests improve robustness but incur delay; redundancy and conservative decoding reduce throughput; and certified or worst-case–oriented designs often sacrifice clean-condition accuracy. Because semantic representations propagate across the pipeline, defensive choices made at the encoder or channel level directly affect downstream task performance. As a result, security cannot be optimized in isolation but must be balanced against system-level performance objectives.

% While this coupling is often viewed as a limitation, it also presents an opportunity to reason about semantic security in a principled, quantitative manner. A practical way to do so is through \emph{operating envelopes}. An operating envelope characterizes the achievable region of task utility as a function of security risk, latency, rate, and energy under explicit channel and adversary budgets. Within this view, defense mechanisms such as detector thresholds, semantic bitrate, redundancy, and model selection act as control variables, while channel conditions and attacks appear as disturbances. Offline sweeps over these controls yield Pareto frontiers that expose robustness--efficiency tradeoffs, allowing designers to identify operating points that meet service-level objectives rather than maximizing a single metric.

% Once such envelopes are established, runtime behavior becomes a policy-selection problem rather than ad hoc tuning. The system maintains a small set of validated operating points, each associated with explicit guarantees on semantic accuracy, delay, and fallback behavior. Online telemetry, such as channel state, detector confidence, and budget utilization, then drives transitions among these points. This approach enables graceful degradation under stress, ensures predictable behavior under attack, and prevents defensive mechanisms from silently exceeding latency or energy budgets.

% From an evaluation and governance perspective, operating envelopes provide a common language for reporting robustness. Instead of single-point results, systems should report expected task utility and security risk at fixed latency and energy constraints, together with abstention rates and fallback frequencies. Provenance metadata binding outputs to model versions, channel descriptors, and knowledge snapshots ensures that operating points are auditable and comparable across deployments. More broadly, operating envelopes offer a natural interface for benchmarking and standardization, as they decouple robustness claims from specific architectures while preserving budget-aware semantics.

% Key research challenges include automated construction of operating envelopes for complex pipelines, learning control policies that adapt thresholds under uncertainty while respecting hard budgets, and standardizing semantic corruption and over-the-air attack models so that envelopes are portable across studies. Addressing these challenges is essential for moving from isolated robustness gains to deployable, contractable semantic security.

% \subsection{Deployment Under Resource and Deadline Constraints}
% SemCom systems are often deployed under strict real-time constraints, where latency, energy, and computational budgets are as binding as security requirements. In such settings, even modest defensive overheads, such as additional detection passes, generative correction, redundancy, or model switching, can cause deadline violations that directly translate into semantic loss or task failure. Consequently, the primary deployment challenge is not average-case robustness, but preserving semantic integrity under tight deadlines and tail-latency behavior.

% Resource constraints interact with security mechanisms in non-uniform ways. Detection and purification costs depend on channel conditions and adversarial pressure; generative modules and ensemble decoding are often only partially interruptible; and shared accelerators introduce contention across flows. Naive backpressure or best-effort scheduling can propagate stalls across layers, causing oscillations between under-protection and overload. In the worst case, defensive mechanisms intended to improve robustness may instead degrade system-level reliability by triggering missed deadlines or cascading queue buildup.

% A practical deployment principle is \emph{deadline-first defense}. The system admits defensive actions only when sufficient slack remains to meet end-to-end latency constraints; otherwise, it degrades gracefully to lower-cost semantic representations or fallback policies. Examples include switching to compressed or lower-precision semantic codes, invoking early-exit heads in multi-stage decoders, or reusing cached semantic outputs when confidence permits. Safety- or mission-critical flows are assigned priority lanes with reserved compute and airtime, ensuring that defensive actions for best-effort traffic do not compromise critical semantics.

% Effective deployment further requires tight integration between scheduling, resource governance, and semantic policy. Per-flow budgets for compute, memory, and airtime should be enforced through lightweight governors, while telemetry emphasizes tail behavior (e.g., p95 and p99 latency, deadline miss rates) rather than averages. Long-lived models are pinned to devices to avoid cold starts, channel features and semantic priors are cached where possible, and blue--green rollouts are used for model or knowledge updates to prevent service interruption. Micro-batching and speculative decoding are employed only when their added delay is explicitly accounted for in the operating envelope.

% From an evaluation standpoint, deployment realism must be reflected in experimental design. Robustness claims should be reported under explicit deadline and power budgets, with stress tests that include bursty traffic, time-varying channels, and partial resource contention. Security improvements that rely on rare but expensive defensive paths should quantify their impact on tail latency and service-level objectives. These practices are not intended as a reference architecture, but as design principles for aligning semantic robustness with real-time system constraints.

% Overall, deployment under resource and deadline constraints reinforces a central lesson of semantic security: defenses must be engineered as budget-aware system components rather than standalone mechanisms. Only by explicitly accounting for deadlines, tail behavior, and shared resources can SemCom systems achieve robustness that is both meaningful and operationally sustainable.

% \subsection{Certification and Verifiable Robustness in Semantic Communications}
% Certification aims to provide \emph{provable guarantees} on system behavior under explicitly defined threat models. In the context of SemCom, this means certifying task-level semantic integrity, such as intent correctness, control-action validity, or semantic similarity, against adversarial perturbations that are physically and semantically realizable. Unlike conventional AI settings, SemCom systems must certify robustness across a stochastic encoder–channel–decoder pipeline, where uncertainty arises not only from adversarial inputs but also from wireless fading, interference, retransmissions, and protocol dynamics.

% Despite recent progress in randomized smoothing, Lipschitz bounding, and linear-relaxation–based verification, certified SemCom remains in its infancy. Existing certification techniques were developed largely for static, model-centric settings, and their assumptions rarely align with the physics, randomness, and feedback inherent to SemCom systems. As a result, certification in SemCom should be viewed as an aspirational but necessary capability, rather than a mature tool that can be directly applied.

% A central difficulty lies in the mismatch between standard certification tools and SemCom realities. Norm-bounded perturbations at the model input do not map cleanly to over-the-air adversaries constrained by power, bandwidth, and spectral masks. Channel randomness, HARQ, and adaptive rate control violate worst-case assumptions commonly used in certification, while semantic utility is often non-smooth or discrete, complicating Lipschitz-based bounds. Consequently, certificates derived for isolated encoders or task heads rarely compose into meaningful end-to-end guarantees once channel effects and system policies are included.

% A pragmatic path forward is to tailor certification to the \emph{physics and semantics} of communication systems. First, adversary models should be expressed in over-the-air terms—such as SNR bins, error vector magnitude (EVM), time–frequency–localized interference, or bounded semantic edit distances—rather than generic $\ell_p$ balls. Second, certification should target representations where semantic utility is smoother and more stable, such as encoder latents or task heads, and be paired with band-limited preprocessing so that certified threat sets align with realizable wireless perturbations. Third, certification should embrace abstention and fallback as first-class outcomes: when guarantees cannot be maintained within budget, the system should explicitly signal uncertainty or degrade semantics in a controlled manner.

% Equally important is treating certificates as \emph{runtime artifacts} rather than offline proofs. Certified regions, confidence radii, and validity windows should be attached as provenance metadata to semantic outputs, binding decisions to specific model versions, channel states, and knowledge snapshots. System policies can then gate high-cost defensive actions or safety-critical actuation on certificate status, enabling dynamic tradeoffs between robustness, latency, and energy. Reporting certified performance as operating envelopes—semantic utility versus channel condition, deadline, and power—provides a more honest and deployable characterization than single-point robustness claims.

% Open research directions include certifying end-to-end JSCC under channel randomness, extending guarantees to multi-antenna and multi-user settings, and developing smooth semantic surrogates that better align with task-level metrics. Incremental advances, such as cached or streaming certificates and composition rules that lift local guarantees to system-level assurances, will be critical for making certification a practical component of deployed SemCom systems.

% \subsection{Cross-Layer Threats and Defense Composition}
% A central limitation of existing defenses is that semantic failures often arise from the \emph{composition} of otherwise admissible perturbations across multiple system components. While Sections~\ref{sec:AI-security} and~\ref{sec:semcom-defenses} analyzed threats and defenses at individual layers, practical adversaries are not confined to a single interface. Small manipulations applied jointly at the source, channel, knowledge, or coordination layers can combine to produce large semantic degradation, even when each layer operates within its assumed threat model. As a result, end-to-end semantic security cannot be inferred from the robustness of isolated components.

% These cross-layer failures are typically caused by mismatched assumptions rather than by broken mechanisms. Encoder-level defenses often assume fixed channels and synchronized context. Channel-level defenses treat semantic decoders as stable functions. Knowledge and network defenses reason about integrity and trust independently of signal-level uncertainty. When deployed together, these assumptions need not hold simultaneously, allowing perturbations to propagate and interact in ways that were not exercised during training or evaluation. Importantly, this subsection does not argue for a new class of defenses. Instead, it highlights a gap between how defenses are \emph{validated} and how systems \emph{fail}. Most robustness guarantees do not compose: adversarial training, channel hardening, and trust mechanisms are typically evaluated under single-layer perturbations and static contexts. When combined, their guarantees may weaken or even interfere, producing brittle behavior that is difficult to diagnose post hoc.

% From an engineering standpoint, mitigating composed attacks requires system-level controls rather than deeper specialization at individual layers. One practical step is to evaluate robustness against \emph{joint perturbation budgets}, even if coarsely defined, to expose interaction effects early. Another is to monitor semantic consistency across layers by comparing multiple signals, such as encoder confidence, channel-induced uncertainty, and knowledge plausibility, and using disagreement as a trigger for conservative system policies. These mechanisms do not require precise attack attribution; they aim only to prevent silent semantic failure.

% Equally important is policy-level coordination. Detectors, robustness estimates, and trust signals should feed into a unified control policy governing semantic rate, redundancy, model selection, or abstention. Treating these signals independently risks underreaction to composed threats or overreaction to benign noise. Viewing defense as a control problem aligns naturally with the operating-envelope perspective introduced earlier in this section.

% Defending against cross-layer and composed attacks remains a \emph{structural challenge}, rooted in the absence of established methodologies for specifying joint threat models and for reasoning about how local guarantees interact under adaptation and feedback. Addressing this challenge is essential for moving from component-wise robustness to deployable, end-to-end semantic security, and it motivates evaluation frameworks and certification practices that reflect system-level behavior rather than isolated defenses.


% Section~\ref{sec:semcom-defenses} framed semantic security as a system-level allocation problem: protection must be applied where attacks enter, defensive signals should drive policy rather than operate in isolation, and operational decisions must be bound to verifiable system states. While surveyed a broad range of AI-inspired defense mechanisms across the SemCom pipeline, a central challenge remains: \textbf{how to operationalize these defenses as repeatable, auditable, and composable system behaviors}.

% The difficulty is not the absence of defense techniques, but the gap between how they are evaluated in isolation and how SemCom systems are deployed in reality. Mismatches between training and deployment conditions, weak provenance and governance, and the lack of operating envelopes that price robustness against latency, rate, and energy continue to limit the reliability of existing designs. Real-time constraints, heterogeneous hardware stacks, and over-the-air uncertainty further amplify these gaps, and robustness guarantees established at individual components rarely compose into end-to-end semantic security.

% This section takes a pragmatic step from principles to practice. We examine how security–utility tradeoffs should be quantified, how detection and robustness signals can be converted into system-level policies, and how robustness claims can be made portable through certification, provenance, and standardized semantic budgets. Rather than introducing new defense primitives, the emphasis is on engineering controls and evaluation frameworks that make semantic defenses deployable, verifiable, and comparable across systems.

% Section~\ref{sec:semcom-defenses} argued for treating robustness as a system allocation problem: spend protection where attacks enter, use signals to drive policy, and bind decisions to verifiable states. What remains hard is not another defense trick but turning that stance into repeatable engineering. The field still wrestles with mismatches between training and deployment, thin provenance and governance, and the fact that many results do not come with operating envelopes that price robustness against latency, rate, and energy. Real-time constraints and heterogeneous stacks amplify these gaps, and local guarantees seldom compose into end-to-end assurances.

% This section takes a pragmatic step from principles to practice. We surface where present techniques reach their limits, articulate controls that can be deployed now, and outline research that would make defenses auditable and contractable. The emphasis is on quantifying tradeoffs, converting detectors into policies, binding outputs to models and knowledge states, and standardizing semantic budgets and OTA conditions so that robustness claims are portable rather than anecdotal.

% \subsection{Tradeoff in Security and Task Accuracy}
% Security mechanisms in SemCom interact tightly with task accuracy, latency, rate, and energy. Tighter detectors raise false positives that remove useful content, abstention and re-requests increase delay, redundancy lowers throughput, and certification or conservative decoding can reduce clean accuracy. Because upstream choices at the encoder or on the channel propagate to the task head, the design objective is to position the system on a stable operating envelope where accuracy, security risk, rate, latency, and energy are jointly acceptable rather than optimized in isolation.

% A useful formulation treats defense as a control problem. Detector thresholds, abstention policies, and joint source–channel coding redundancy act as control actions, while channels and adversaries appear as disturbances. Offline sweeps over these actions produce Pareto frontiers that reveal utility–cost tradeoffs under specified channel and attacker budgets. From these maps, the system selects a small set of operating points tied to service levels, each with clear specifications for sensitivity, fallback behavior, and redundancy. Online selection then becomes a policy problem driven by telemetry and budget constraints rather than ad hoc tuning.

% Evaluation and governance must align with this framing. Outputs should be bound to verifiable states such as model version, channel descriptors, and knowledge snapshots so that rollback and containment are safe. Reporting should present expected security risk at fixed latency and energy budgets, not only single operating points. Research priorities include automated construction of envelopes, online policies that learn thresholds from feedback while honoring budgets, and standardized semantic corruption budgets that make operating points comparable across studies.


% \subsection{Resource Constraint at Deployment}
% Real-time deployment exposes security mechanisms to deadline pressure and tail behavior. Even modest amounts of extra detection, abstention, or redundancy consume compute and airtime; a small fraction of slow paths can negate average-case gains. Heterogeneous accelerators, co-tenancy with other tasks, and asynchronous model or knowledge updates complicate timing further, and missed deadlines translate directly into semantic loss.

% The scheduling problem is difficult because costs vary with channel state and adversarial pressure, many decoders are only partially interruptible, and queues can build faster than they drain. Naive backpressure pushes stalls across layers, and without deadline aware control the system oscillates between under-protection and overload, producing both false negatives and missed service levels.

% A practical design is deadline first. The system admits work only when the remaining budget can meet the end-to-end deadline; otherwise it degrades gracefully to compressed semantics, lower precision heads, or cached outputs. Safety critical flows receive priority lanes with reserved compute, and heads on the hot path provide early exits so that partial results are available when time is tight. Long lived models are pinned to devices to avoid cold starts, channel features are precomputed and cached, and micro-batching is used only when added delay is acceptable. Per-flow compute and airtime budgets are enforced with simple governors, tail focused telemetry such as p95, p99, and deadline miss rates is collected, and model or knowledge updates follow blue–green rollouts to avoid pauses. Evaluation scenarios include bursty traffic and time-varying channels, and results report security risk and task utility at fixed deadlines and power budgets rather than averages alone.


% \subsection{Certification of Defensive SemCom}
% Certified methods aim to provide provable robustness guarantees under explicit threat models. In SemCom, this means certifying task-level semantic fidelity (e.g., intent classification, caption utility, control-action correctness) against physically realizable perturbations that occur over the air or as bounded semantic edits upstream. Unlike standard vision/NLP settings, the encoder–channel–decoder pipeline is stochastic, the attacker budget is often power- and spectrum-constrained. Certificates therefore must couple waveform budgets (e.g., EVM, band-/time-limited distortions, SNR bins) with semantic budgets (task loss, meaning-preserving distortions), and report guarantees that factor rate, latency, and energy. Therefore, the defense in SemCom system needs to consider not only the adversarial injection (perturbations in source data), but also the intermediate noise from wireless channel.

% The central difficulty is mismatch of norms and models. $\ell_p$ bounds at the encoder input do not map cleanly to OTA-constrained adversaries; fading and HARQ induce randomness that breaks worst-case assumptions; and utility is often non-Lipschitz in raw samples. Existing techniques—randomized smoothing (including denoise/filtered variants), Lipschitz and LiRPA (linear relaxation–based propagation) bounds—cover parts of the stack but rarely the encoder–channel–decoder composition. Moreover, the certification is sample-wised and heavily computation cost to derive a fine-grained certified region.

% A practical path is to tailor certificates to SemCom’s physics and semantics. (i) \textit{Model the attacker in OTA terms}: certify against power-, bandwidth-, and time–frequency–localized budgets, not generic $\ell_p$ balls; for discrete attacks (e.g., MCS flips), certify policy invariants (“decision unchanged within SNR bin $b$”). (ii) \textit{Certify at the right representation}: apply smoothing or Lipschitz control to encoder latents or task heads where utility is smoother; pair with bandlimited prefilters so the certified threat set matches radios. (iii) \textit{Make certificates first-class runtime artifacts}: attach per-packet certificate summaries (radius/budget, sigma, bound type, validity window) as provenance metadata; gate high-cost fallbacks on certificate failure. (iv) \textit{Report envelopes, not points}: publish certified task utility vs.\ SNR/channel, deadline, and energy; include abstention rates (“certify-or-abstain”) to keep guarantees truthful under time pressure. Promising research directions include certifying end-to-end JSCC with channel randomness, multi-antenna certificates that trade spatial diversity for certified radii, semantic metrics with smooth surrogates amenable to LiRPA, cached/incremental bounds for streaming, and composition rules so local certificates yield system-level guarantees.


% \subsection{Defending Cross-Layer Threats}
% A key open challenge in semantic communication (SemCom) security is that semantic failures often emerge only from the interaction of multiple components, rather than from any single module in isolation. While existing defenses largely target individual layers—such as the encoder/decoder, semantic representations in transit, the knowledge base, or network coordination—adaptive adversaries can compose manipulations across these layers to induce severe semantic degradation under system-level constraints. This makes end-to-end (E2E) security an emergent property of the system, rather than a separable defense layer.

% A small number of studies illustrate this difficulty. Prior work shows that jointly optimized perturbations applied across the source, wireless signal, and task pipeline can significantly degrade semantic outcomes while leaving conventional metrics largely unaffected. Other efforts attempt to address such risks via end-to-end robust training or by embedding security primitives directly into semantic encoder–decoder mappings. However, these approaches are typically task-specific, computationally expensive, and tightly coupled to particular system assumptions, limiting their general applicability.

% The core challenge is therefore not the absence of isolated defenses, but the lack of principled methods to \emph{compose} defenses across layers. In practical SemCom systems, encoder/decoder robustness, representation-level protection, knowledge-base integrity, and network-level trust mechanisms are developed largely independently, with no guarantees that their combination yields meaningful end-to-end security. Moreover, control-plane components—such as model updates, orchestration services, and training interfaces—introduce additional cross-layer dependencies that are poorly captured by existing threat models.

% Promising future directions include (i) unified cross-layer threat models that explicitly capture how semantic perturbations propagate across components; (ii) modular defense composition frameworks that provide system-level guarantees from independently designed defenses; and (iii) lightweight runtime monitoring and control mechanisms that detect semantic inconsistencies across layers and trigger adaptive responses. Addressing these challenges is essential for moving from component-wise robustness to trustworthy, end-to-end secure semantic communication systems.


%%\section{Evaluation Frameworks for Semantic Communication Security}\label{sec:evaluation}
%%Evaluating SemCom security requires an integrated methodology that extends beyond traditional wireless or AI metrics. Traditional metrics focus on bit-level fidelity or model accuracy under independent and identically distributed (i.i.d.) inputs, whereas SemCom involves complex interactions across encoders, channels, knowledge modules, and downstream tasks. As a result, robustness and utility must be assessed jointly, under system constraints and adversarial conditions. This section outlines the emerging principles, metrics, and experimental frameworks for evaluating secure SemCom systems, with emphasis on standardizing semantic robustness evaluation under constrained, adversarial, and deployment-realistic conditions. We begin by examining foundational evaluation metrics and benchmarking needs for semantic security, followed by threat simulation and red-teaming approaches to probe practical vulnerabilities. We conclude with a discussion of real-world testbeds and deployment validation strategies.

\subsection{Evaluation Metrics and Benchmarking Gaps}
The evaluation of security in SemCom systems requires a fundamental rethinking of what constitutes robustness, utility, and performance. Traditional metrics such as bit error rate (BER), SNR, or downstream task accuracy offer limited visibility into the security posture of SemCom pipelines, especially under adversarial conditions. Unlike classical norm-bounded robustness metrics in machine learning \cite{carlini2017towards}, adversarial budgets in SemCom reflect semantic corruption, protocol behavior, and physical-layer constraints. This calls for a shift toward \textbf{semantic robustness}, an evaluation axis that measures degradation in meaning preservation, task utility, or reconstruction fidelity under worst-case semantic perturbations or cross-layer interference. For instance, in visual SemCom, degradation can be quantified via mean intersection over union (mIoU) or classification accuracy under semantic perturbation, while in language tasks, BLEU or semantic similarity scores may better reflect task failure. Fig.\ref{fig:result-safeguraded} takes the metric of BLEU to evaluate the reliability performance under different channel conditions \cite{liang2025safeguarded}.

\begin{figure}[t!]
\centering
\includegraphics[width=0.70\linewidth] {figures/result-safeguarded-AI.pdf}
\caption{BLEU (1-gram) scores for the proposed secure SemCom framework with varying thresholds ($\tau =0.5, 0.6, 0.7$) vs. DeepSC \cite{liang2025safeguarded}. The parameter $\tau$ is the safeguarded threshold guaranteed in the proposed framework. DeepSC is a traditional SemCom framework with no consideration of security.}
\label{fig:result-safeguraded}	
\end{figure}

Semantic robustness should also account for context dependence and knowledge misalignment \cite{chaccour2024less}, where identical transmitted representations may yield divergent interpretations due to corrupted priors or desynchronized knowledge bases. For example, attacks may not directly perturb the transmitted signal but instead induce semantic failure by poisoning the receiver’s grounding assumptions. Benchmarks should reflect this cross-domain fragility by modeling both data-space and knowledge-space divergence. All evaluation pipelines should support dual reporting under benign and adversarial conditions to expose hidden robustness–utility tradeoffs that would otherwise remain latent under average-case testing.

Beyond robustness, security evaluations should quantify \textbf{semantic leakage}, which reflects the extent to which transmitted representations inadvertently reveal private or structured information about the source input \cite{nasr2019comprehensive,liu2021machine,elliott2022ai}. Leakage can be measured via mutual information, inversion success rates, or recoverability of sensitive attributes from latent codes. For systems employing modular or cross-task semantic encoding, leakage may also span unrelated downstream applications, requiring broader auditing.

In deployment scenarios, \textbf{operational tradeoffs} connect robustness with system viability. These include latency–robustness curves, semantic fidelity versus throughput, and energy per bit of meaning \cite{saad2019vision,zhu2020toward,zhang2025resource,hua2025bandwidth,ma2025power,liu2025joint}. Semantic envelope violation rates, \textit{i.e.}, instances where performance falls below acceptable thresholds under attack, are especially useful for quantifying resilience limits in constrained environments such as edge devices or time-critical inference pipelines. In particular, metrics such as semantic envelope violation rates—instances where system outputs fall below predefined semantic fidelity thresholds under adversarial stress—highlight brittle operational regions and enable quantification of robustness boundaries. Similarly, latent trust drift, where decoder predictions diverge gradually due to upstream semantic desynchronization or poisoned priors, can be monitored to trigger adaptive defenses or trust recalibration protocols. For example, Fig.\ref{fig:result-overhead} examines the time overhead and communication overhead of training reliable SemCom coding models \cite{shen2023secure}. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.70\linewidth] {figures/simulation-2.png}
\caption{Time overheads and communication overheads of reliable training method for secure SemCom\cite{shen2023secure}.}
\label{fig:result-overhead}	
\end{figure}

Despite these needs, current SemCom evaluations remain fragmented and ad hoc \cite{getu2025semantic}. Most reuse task-oriented metrics from AI or wireless domains without addressing SemCom-specific risks. The field urgently requires reproducible, open-source benchmark suites that simulate realistic attacker models, environmental variations, and cross-layer semantics. Only with such foundations can future work offer rigorous guarantees and practical resilience at scale. To capture SemCom-specific risks under realistic stress, static metrics should be complemented with adaptive adversarial evaluation, as elaborated in the next subsection

\subsection{Threat Simulation and Red-Teaming}
While static benchmarks and norm-bounded attacks provide valuable baselines, they fail to capture the adaptive, layered nature of real-world adversaries. Red-teaming fills this gap by simulating intelligent, feedback-driven agents that dynamically probe, manipulate, and stress-test SemCom  
pipelines under realistic conditions \cite{morris2020textattack,zhao2023evaluating,brundage2020toward}.

\textbf{Red-teaming agents} adapt their strategies based on observed system responses, such as retransmission patterns, decoding confidence, or semantic drift. For instance, a semantic-aware jammer may evolve its interference by monitoring task failure rates, while a gray-box adversary may exploit repeated queries to reconstruct latent embeddings or trigger meaning misalignment. These agents can operate across layers, such as coordinating encoder poisoning, channel perturbations, and knowledge-base desynchronization, to induce emergent failures that span semantic, protocol, and physical layers—failures that remain latent in isolated testing. Effective implementations may rely on techniques such as reinforcement learning, adversarial co-training, or meta-learning to co-evolve with system defenses \cite{goyal2023survey}.

\textbf{Threat roles and surfaces} vary in observability and access: white-box agents emulate insider threats with full model access; gray-box attackers observe intermediate features or metadata; black-box adversaries interact only with system inputs and outputs \cite{goyal2023survey,papernot2017practical}. Attack surfaces span semantic-aware jamming, backdoor insertion, knowledge poisoning, privacy leakage, and coordinated misinformation in multi-agent settings. A modular red-teaming framework should support diverse attacker profiles and allow composition of complex, multi-phase campaigns that reflect real-world threat evolution.

\textbf{Integrated evaluation} embeds red-teaming agents into training, adaptation, or runtime inference to reveal resilience under dynamic pressure. Defenses such as decoder switching, abstention, or knowledge re-synchronization can be stress-tested using runtime triggers like semantic mismatch, latent trust drift, or envelope violations \cite{meng2025securesemcom}. Beyond degrading performance, red-teaming enables \textit{semantic risk auditing}—a diagnostic process that identifies brittle input modalities, fragile concept classes, and cascading failure paths. These insights support the development of semantic risk budgets that quantify acceptable degradation bounds under adversarial stress, particularly for safety-critical applications such as autonomous driving, remote surgery, or multi-agent coordination.

Ultimately, red-teaming is not a replacement for theoretical analysis or benchmark testing but a necessary complement. By exposing emergent, cross-layer vulnerabilities that elude static analysis, red-teaming provides a pathway toward more trustworthy, resilient SemCom systems. Future work should prioritize open-source red-teaming toolkits tailored to SemCom, incorporating domain-specific artifacts such as latent codes, shared priors, and task-conditioned decoders. However, even the most sophisticated simulations should ultimately be validated under physical constraints, motivating real-world testbed deployments.

\subsection{Real-World Testbeds and Deployment Studies}
Simulation and red-teaming offer powerful abstractions for evaluating SemCom security. However, validating resilience under real-world constraints requires deployment-centric testbeds that expose the unpredictability of physical hardware, asynchronous control loops, and imperfect communication channels.

\textbf{Semantic observability} is central to effective deployment studies. Unlike conventional wireless testbeds that focus on throughput, delay, or error rates, SemCom evaluation requires introspection into latent code distributions, semantic drift, decoder disagreement, and knowledge desynchronization. Emerging 6G/O-RAN platforms \cite{bonati2021intelligence,polese2023understanding}, augmented with software defined radios (SDRs), xApps, and edge AI accelerators, provide partial support for this layered introspection. These platforms should be extended to monitor high-level behaviors such as task-level degradation under semantic mismatch and adversarial drift. For example, Fig.\ref{fig:result-implenmentation} shows a simple SemCom platform based on SDR-based LoRa system, which includes two computers and USRPs to perform practical semantic coding and data transmission over a wireless link \cite{ma2024implementation}. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.80\linewidth] {figures/simulation-implementation.png}
\caption{Semantic communication on SDR-based LoRa communication platform \cite{ma2024implementation}.}
\label{fig:result-implenmentation}	
\end{figure}

Testbeds expose \textbf{practical system constraints} that often go unnoticed in simulation. Knowledge re-synchronization mechanisms may fail under lossy control channels or when agents are asynchronously updated. Redundancy-based defenses, such as ensemble decoding or semantic voting, may conflict with stringent real-time latency constraints typical of edge environments. Practical issues such as hardware timing violations, adaptation delays, and resource contention often emerge as performance bottlenecks during deployment and must be explicitly profiled.

Beyond synthetic benchmarks, testbeds allow \textbf{cross-domain robustness evaluation} across realistic and heterogeneous settings, ranging from remote robotic control and telehealth to rural IoT deployments \cite{qiu2018can}. These domains introduce asymmetric vulnerabilities: low-power encoders at the edge may rely on powerful, semantically informed decoders in the cloud, resulting in one-sided failure modes when semantic codes are distorted or desynchronized. Edge–cloud heterogeneity, link asymmetry, and mobility further stress semantic security under real-world operating envelopes.


\begin{table*}[!t]
\centering
\caption{Deployment-Aware Evaluation Dimensions for Semantic Communication Security.}
\label{tab:evaluation-framework}
\begin{tabular}{|p{2.5cm}|p{3.5cm}|p{5cm}|p{5cm}|}
\hline
\textbf{Evaluation Goal} & \textbf{Security Objective} & \textbf{Evaluation Method} & \textbf{Representative Threats and Failure Modes} \\
\hline
\textbf{Semantic Robustness} & Meaning preservation and task utility under adversarial semantic perturbations & Semantic fidelity metrics, adversarial perturbation tests, semantic envelope violation rates & Knowledge misalignment, decoder drift, semantic corruption \\
\hline
\textbf{Semantic Leakage} & Privacy exposure from latent representations or shared knowledge & Mutual information analysis, inversion success rate, sensitive attribute recovery & Latent inversion, encoder leakage, cross-task information leakage \\
\hline
\textbf{Operational Resilience} & Tradeoffs between robustness, latency, and energy under adversarial and runtime constraints & Latency–robustness curves, energy per bit of meaning, graceful degradation tests & Time-critical failures, resource exhaustion, edge deployment stress \\
\hline
\textbf{Threat Adaptability} & System behavior under adaptive, multi-phase adversaries & Adaptive red-teaming agents, multi-stage and feedback-driven stress testing & Gray-box jammers, encoder poisoning, semantic desynchronization \\
\hline
\textbf{Deployment Robustness} & Resilience under real-world hardware, protocol, and update constraints & SDR-based testbeds, fault injection, runtime observability and monitoring & Semantic-aware jamming, asynchronous updates, decoder disagreement \\
\hline
\end{tabular}
\end{table*}


\textbf{Controlled fault injection} provides additional levers for testing adversarial resilience. SDR-based waveform injection can simulate semantic jamming at the physical layer. Compromised agents can be used to poison models or propagate misinformation through shared knowledge graphs. These setups further support fallback evaluations, including abstention, human-in-the-loop verification, and automated triggers for semantic anomalies.
To enable reproducible and modular evaluation, future efforts should prioritize open-source testbeds that integrate semantic communication pipelines, red-teaming agents, and runtime observability. Platforms such as Powder-RENEW \cite{powderrenew}, B5G Playground \cite{b5gplayground}, OpenAirInterface \cite{oai2023}, ARA \cite{ara2020testbed}, and RISE-6G \cite{rise6g2023} provide promising foundations for SemCom-aware security experimentation and system-level validation.

\subsection{Lessons Learned}
In summary, bridging the design and deployment of secure semantic communication necessitates a holistic, system-aware approach that moves beyond isolated model hardening to address the interdependencies between semantic fidelity, robustness, latency, and resource constraints. Practical deployment of secure SemCom calls for the need for security-utility operating envelopes to manage tradeoffs under real-world conditions. Besides, table~\ref{tab:evaluation-framework} summarizes the key evaluation dimensions discussed in this section, highlighting metrics and methodologies for assessing SemCom security under adversarial and deployment-realistic conditions.

This section reveals that securing SemCom is fundamentally a co-design challenge, requiring tight integration of AI defenses with communication protocols, knowledge management, and network coordination. Success depends not only on advancing robustness techniques but also on developing adaptive, lightweight assurance mechanisms that can operate within strict operational envelopes, supported by continuous adversarial evaluation and deployment-focused validation. In this way, SemCom systems can achieve the resilience and trustworthiness required for real-world, safety-critical applications.



%In summary, a comprehensive evaluation framework for SemCom security must integrate structured metrics (Section VI.A), dynamic threat simulation (Section VI.B), and real-world deployments. 
%, as summarized in Table \ref{tab:evaluation-framework}. Only by combining introspective, adversarial, and physical perspectives can we ensure that SemCom systems remain robust and trustworthy in practice.

% \section{Evaluation Frameworks for Semantic Communication Security}\label{sec:evaluation}
% Evaluating the security of SemCom systems requires fundamentally different methodologies than those used in traditional wireless or standalone AI settings. Unlike classical metrics that emphasize bit-level fidelity or model accuracy under independent and identically distributed (i.i.d.) inputs, SemCom systems operate across layers, where meaning is formed by the interplay between encoder-decoder pairs, channel characteristics, shared knowledge, and inference tasks. As such, robustness and utility must be assessed jointly and holistically, taking into account system constraints, attack surfaces, and task goals. 

% This section outlines the emerging principles, metrics, and experimental frameworks for evaluating secure SemCom systems, with emphasis on standardizing semantic robustness evaluation under constrained, adversarial, and deployment-realistic conditions. We begin by examining foundational evaluation metrics and benchmark needs for semantic security (A), followed by threat simulation and red-teaming approaches to probe practical vulnerabilities (B), and conclude with a discussion of real-world testbeds and deployment validation strategies (C).

% \subsection{Evaluation Metrics and Benchmarks}
% Despite significant progress in SemCom systems, the evaluation of their security remains insufficiently defined. Most existing studies assess performance using isolated task-level metrics, such as BLEU scores or classification accuracy, or rely on communication-centric indicators such as PSNR or bit error rate. While informative in limited contexts, these metrics do not capture the defining characteristics of secure SemCom: robustness under adversarial perturbations, dependence on shared knowledge and context, and operation under stringent latency, energy, and resource constraints. As a result, comparisons across designs are difficult, and deployment-relevant security guarantees remain elusive.

% To support reproducible, comparable, and system-level evaluation, semantic security must be assessed through a structured set of metrics that jointly reflect meaning preservation, adversarial resilience, and operational feasibility. We organize these metrics into four complementary categories.

% \textbf{Semantic utility} metrics form the foundation of SemCom evaluation. At their core is the question of whether the intended meaning is preserved under operational conditions. In task-driven settings, this is often measured through task accuracy, such as classification correctness or decision success. For language, vision, and multimodal communication, semantic similarity metrics including BLEU, ROUGE, CIDEr, or learned embedding-based scores such as CLIP similarity are commonly used to quantify reconstruction fidelity. In goal-directed or interactive systems, intent preservation becomes critical, requiring evaluation of whether downstream actions or inferred objectives align with the original communicative goal. In safety-critical deployments, abstention or fallback behavior must also be accounted for, as the ability to withhold decisions under low confidence can be as important as correctness itself. Importantly, semantic utility should be reported under both benign and adversarial conditions to expose robustness degradation rather than average-case performance.

% Beyond utility, \textbf{robustness and security metrics} are essential for characterizing resistance to semantic attacks. Rather than relying on classical $l_p$-norm–bounded perturbations, SemCom robustness must be defined with respect to adversarial budgets that reflect semantic corruption, channel power constraints, or poisoning intensity. Semantic robustness curves, which plot task utility against adversarial strength, provide a concise view of degradation behavior. Worst-case semantic distortion captures the maximum loss in utility under constrained attacks, offering a conservative security measure. At the representation level, latent code perturbability quantifies the sensitivity of semantic decoding to perturbations in learned embeddings. Privacy-oriented evaluation further requires measuring semantic leakage, such as the success of sensitive attribute inference or mutual information between latent representations and private data. These metrics reflect the fact that semantic security is as much about limiting inference as it is about preserving correctness.

% Because semantic defenses operate within real systems, \textbf{operating envelope metrics} are equally critical. Security mechanisms inevitably interact with latency, throughput, and energy budgets, and these interactions must be explicitly evaluated. Latency–robustness tradeoffs reveal how defensive actions affect deadline miss rates or tail latency. Throughput versus semantic fidelity captures how robust encoding and retransmission policies scale under attack or interference. Energy per bit of meaning provides a unified measure of communication and computation cost relative to semantic utility, particularly relevant for edge and IoT deployments. Finally, adversarial envelope violation rates quantify how often system performance falls below application-specific semantic thresholds under constrained attacks. Visualizing these relationships as operating envelopes, for example task accuracy as a function of SNR and adversarial power, enables system designers to reason about acceptable operating regions rather than single-point performance.

% Despite these emerging principles, \textbf{benchmarking practice} in secure SemCom remains fragmented. Most evaluations rely on isolated datasets such as CIFAR-10 or COCO with offline corruption models, neglecting over-the-air effects, multi-agent interaction, and adaptive adversaries. There is currently no public benchmark suite designed specifically for semantic communication security that incorporates semantic attacks, cross-layer faults, or dynamic knowledge states. Moreover, many simulation environments abstract away realistic wireless behavior, adversarial scheduling, and evolving knowledge graphs, limiting their relevance to deployment.

% Addressing these gaps requires the development of SemCom-native benchmarks that span image, speech, and text modalities with explicit semantic goals and threat scenarios. Such benchmarks should integrate channel simulators capable of modeling adversarial fading, semantic jamming, and protocol-aware perturbations, alongside standardized evaluation pipelines that jointly measure semantic fidelity, robustness, delay, and resource consumption. Establishing these benchmarks is a prerequisite for meaningful comparison across defense strategies and for translating semantic security research into deployable systems.


% \subsection{Threat Simulation and Red-Teaming}
% While theoretical threat models and benchmark-driven evaluations have laid the foundation for assessing semantic communication security, they often fall short of capturing the complexity and adaptiveness of real-world adversaries. SemCom systems are exposed to a broad range of vulnerabilities across model, channel, knowledge, and network layers—surfaces that can be exploited individually or in combination. To evaluate system robustness against such multifaceted threats, \textbf{red-teaming} provides a complementary methodology: it simulates intelligent, adversarial agents capable of probing, manipulating, and subverting the semantic pipeline through dynamic, feedback-driven strategies.

% In contrast to static perturbation models, \textbf{adaptive adversarial simulation} reflects a more realistic attack scenario in which the adversary observes system responses and adjusts its tactics accordingly. For example, semantic jammers can be trained to react to partial feedback such as task confidence or retransmission frequency, evolving interference patterns that target vulnerable aspects of the receiver’s inference process. Similarly, gray-box adversaries may query the encoder-decoder interface to extract latent representations, reconstruct decision boundaries, or trigger semantic misinterpretation. These attacks can also be composed across layers: subtle encoder poisoning, coupled with channel-level perturbations and knowledge-base desynchronization, can lead to emergent failures that are hard to detect or attribute. Implementing such red-teaming agents requires the use of reinforcement learning, meta-learned perturbation generators, or adversarial co-training frameworks that co-evolve with the system being tested.

% Effective red-teaming must account for diverse \textbf{threat roles and access levels}. White-box adversaries simulate insider threats or compromised devices with access to model weights and training data. Gray-box attackers reflect partially informed actors who observe intermediate outputs, metadata, or channel state. Black-box adversaries operate solely through input–output interaction, emulating external or over-the-air threats in open deployments. Across these roles, adversaries may target different components: implanting backdoors in model training, performing inference-time evasion, injecting semantic-aware jamming at the physical layer, corrupting or desynchronizing shared knowledge, or propagating misinformation in multi-agent settings. An effective red-teaming framework should allow modular composition of these capabilities and support simulation across a range of configurations, enabling defenders to evaluate not just isolated modules but the system’s layered defenses and fallback strategies in the face of coordinated threats.

% For threat simulation to inform system design and deployment, it must be \textbf{integrated into evaluation pipelines}. This includes injecting adversarial behavior during training, adaptation, or inference, and monitoring the resulting impact on semantic utility, operating envelope violations, and decision confidence. Defenses that respond dynamically—such as abstention, decoder switching, or knowledge re-synchronization—can be evaluated under conditions where attacks adapt in real time. Semantic mismatch rates, disagreement between modules, or observed trust drift can be used as runtime triggers for activating these responses. Red-teaming agents can therefore serve not only as evaluators but as part of a closed-loop simulation ecosystem in which robustness is assessed under dynamic, adversarial feedback.

% Beyond performance degradation, red-teaming also enables \textbf{semantic risk auditing}, a diagnostic process that aims to identify and characterize systemic fragilities. For instance, it can help determine which classes of concepts, tasks, or input modalities are most vulnerable to distortion or leakage, or which combinations of model, channel, and knowledge configurations lead to the most brittle behavior. In safety-critical applications such as autonomous driving or remote control, these insights can guide the formulation of semantic risk budgets—quantitative guarantees on acceptable levels of degradation under known attack budgets. Red-teaming can then be used to validate whether system behavior remains within these contractual bounds, even in the presence of sophisticated adversaries.

% Ultimately, red-teaming is not a replacement for theoretical analysis or static benchmarks, but a necessary complement. It brings an adversarial lens to SemCom evaluation, exposing the subtle interactions and emergent behaviors that arise from AI-native design, layered architecture, and dynamic adaptation. To support reproducibility and progress in this area, future efforts should focus on developing open-source red-teaming frameworks tailored to SemCom pipelines, incorporating artifacts such as latent semantic codes, shared knowledge graphs, and end-to-end task fidelity. Such frameworks will be critical for building secure, adaptive, and trustworthy semantic communication systems.

% \subsection{Real-World Testbeds and Deployment Studies}
% While simulation and red-teaming offer powerful abstractions for evaluating SemCom security, translating these findings into real-world reliability requires deployment-centric validation. Semantic communication systems, with their AI-native encoding, cross-layer interactions, and context-dependent reasoning, behave differently when exposed to the uncertainties, imperfections, and constraints of operational environments. Testbed deployment serves as the bridge between theory and practice, offering a sandbox to evaluate robustness, adaptivity, and system-level behavior under realistic conditions.

% A key requirement for deployment studies is semantic observability across layers. Traditional wireless testbeds focus on physical- or network-layer metrics—throughput, delay, packet error rates. In contrast, semantic communication demands instrumentation capable of tracking high-level representations: latent code distributions, semantic task fidelity, decoder alignment, and knowledge synchronization. Emerging 6G and O-RAN platforms provide partial support for such semantic introspection, especially when integrated with software-defined radios (SDRs), edge AI accelerators, and flexible radio access control. Experimental setups must extend these capabilities to monitor semantic drift over time, detect context mismatches, and correlate adversarial perturbations with task-level degradation.

% Real-world testbeds also reveal deployment challenges hidden in simulation, including hardware constraints, system-level timing violations, and adaptation latencies. For example, knowledge resynchronization mechanisms that work well in simulation may be infeasible when distributed agents have mismatched updates or lossy control channels. Similarly, redundancy-based defenses such as ensemble decoding or semantic voting may conflict with latency budgets in edge environments. Deployment studies expose these conflicts, allowing designers to tune tradeoffs between robustness and resource consumption in context-sensitive ways.

% Testbeds enable cross-domain evaluation, where robustness is assessed across multiple application settings—autonomous driving, remote control, edge intelligence, or telehealth. This allows researchers to test whether proposed semantic encodings, certification methods, or fallback strategies generalize beyond synthetic datasets and single-task benchmarks. In particular, edge–cloud heterogeneity and link asymmetry—such as constrained encoders in rural IoT and powerful decoders at aggregation points—create asymmetrical vulnerabilities that can only be evaluated under realistic communication and computational conditions.

% Moreover, testbed deployments support security-focused fault injection, enabling controlled testing of physical-layer jamming, adversarial inputs, or compromised agents. For instance, adversarial waveforms can be injected over-the-air using SDRs to assess semantic jamming resilience. Model poisoning or desynchronized knowledge bases can be introduced to emulate compromised devices. These experiments make it possible to validate fallback mechanisms such as abstention, re-synchronization, or human-in-the-loop verification under actual operational stress, rather than abstract assumptions.

% To support reproducible research and standardized evaluations, there is a growing need for open-source SemCom testbed platforms that integrate semantic encoders/decoders, adversarial modules, and real-time instrumentation. These platforms should provide modular support for tuning channel conditions, injecting semantic-aware perturbations, and measuring end-to-end task reliability. Initiatives such as the ARA rural testbed, O-RAN-based xApp platforms, or edge AI inference over programmable radio networks represent promising foundations for such SemCom-centric evaluations.

% In summary, real-world testbeds play a critical role in closing the gap between algorithmic robustness and system-level trust. By enabling reproducible, configurable, and domain-relevant experimentation, they ensure that semantic security mechanisms do not remain theoretical constructs but evolve into deployable defenses that can withstand the unpredictability of real-world environments.

==> 7_evaluation.tex <==
\section{Evaluation Frameworks for Semantic Communication Security}\label{sec:evaluation}
Evaluating SemCom security requires an integrated methodology that extends beyond traditional wireless or AI metrics. Traditional metrics focus on bit-level fidelity or model accuracy under independent and identically distributed (i.i.d.) inputs, whereas SemCom involves complex interactions across encoders, channels, knowledge modules, and downstream tasks. As a result, robustness and utility must be assessed jointly, under system constraints and adversarial conditions. This section outlines the emerging principles, metrics, and experimental frameworks for evaluating secure SemCom systems, with emphasis on standardizing semantic robustness evaluation under constrained, adversarial, and deployment-realistic conditions. We begin by examining foundational evaluation metrics and benchmarking needs for semantic security, followed by threat simulation and red-teaming approaches to probe practical vulnerabilities. We conclude with a discussion of real-world testbeds and deployment validation strategies.

\subsection{Evaluation Metrics and Benchmarking Gaps}
The evaluation of security in SemCom systems requires a fundamental rethinking of what constitutes robustness, utility, and performance. Traditional metrics such as bit error rate (BER), signal-to-noise ratio (SNR), or downstream task accuracy offer limited visibility into the security posture of SemCom pipelines, especially under adversarial conditions. Unlike classical $l_p$ norm–bounded robustness metrics in machine learning \cite{carlini2017towards}, adversarial budgets in SemCom reflect semantic corruption, protocol behavior, and physical-layer constraints. This calls for a shift toward \textbf{semantic robustness}, an evaluation axis that measures degradation in meaning preservation, task utility, or reconstruction fidelity under worst-case semantic perturbations or cross-layer interference. For instance, in visual SemCom, degradation can be quantified via mIoU or classification accuracy under semantic perturbation, while in language tasks, BLEU or semantic similarity scores may better reflect task failure.

Semantic robustness must also account for context dependence and knowledge misalignment \cite{chaccour2024less}, where identical transmitted representations may yield divergent interpretations due to corrupted priors or desynchronized knowledge bases. For example, attacks may not directly perturb the transmitted signal but instead induce semantic failure by poisoning the receiver’s grounding assumptions. Benchmarks should reflect this cross-domain fragility by modeling both data-space and knowledge-space divergence. All evaluation pipelines should support dual reporting under benign and adversarial conditions to expose hidden robustness–utility tradeoffs that would otherwise remain latent under average-case testing.

Beyond robustness, security evaluations should quantify \textbf{semantic leakage}, which reflects the extent to which transmitted representations inadvertently reveal private or structured information about the source input \cite{nasr2019comprehensive,liu2021machine,elliott2022ai}. Leakage can be measured via mutual information, inversion success rates, or recoverability of sensitive attributes from latent codes. For systems employing modular or cross-task semantic encoding, leakage may also span unrelated downstream applications, requiring broader auditing.

In deployment scenarios, \textbf{operational tradeoffs} connect robustness with system viability. These include latency–robustness curves, semantic fidelity versus throughput, and energy per bit of meaning \cite{saad2019vision,zhu2020toward,zhang2025resource,hua2025bandwidth,ma2025power,liu2025joint}. Semantic envelope violation rates, \textit{i.e.}, instances where performance falls below acceptable thresholds under attack, are especially useful for quantifying resilience limits in constrained environments such as edge devices or time-critical inference pipelines. In particular, metrics such as semantic envelope violation rates—instances where system outputs fall below predefined semantic fidelity thresholds under adversarial stress—highlight brittle operational regions and enable quantification of robustness boundaries. Similarly, latent trust drift, where decoder predictions diverge gradually due to upstream semantic desynchronization or poisoned priors, can be monitored to trigger adaptive defenses or trust recalibration protocols.

Despite these needs, current SemCom evaluations remain fragmented and ad hoc \cite{getu2025semantic}. Most reuse task-oriented metrics from AI or wireless domains without addressing SemCom-specific risks. The field urgently requires reproducible, open-source benchmark suites that simulate realistic attacker models, environmental variations, and cross-layer semantics. Only with such foundations can future work offer rigorous guarantees and practical resilience at scale. To capture SemCom-specific risks under realistic stress, static metrics must be complemented with adaptive adversarial evaluation, as elaborated in the next subsection

\subsection{Threat Simulation and Red-Teaming}
While static benchmarks and norm-bounded attacks provide valuable baselines, they fail to capture the adaptive, layered nature of real-world adversaries. Red-teaming fills this gap by simulating intelligent, feedback-driven agents that dynamically probe, manipulate, and stress-test SemCom  
pipelines under realistic conditions \cite{morris2020textattack,zhao2023evaluating,brundage2020toward}.

\textbf{Red-teaming agents} adapt their strategies based on observed system responses, such as retransmission patterns, decoding confidence, or semantic drift. For instance, a semantic-aware jammer may evolve its interference by monitoring task failure rates, while a gray-box adversary may exploit repeated queries to reconstruct latent embeddings or trigger meaning misalignment. These agents can operate across layers, such as coordinating encoder poisoning, channel perturbations, and knowledge-base desynchronization, to induce emergent failures that span semantic, protocol, and physical layers—failures that remain latent in isolated testing. Effective implementations may rely on techniques such as reinforcement learning, adversarial co-training, or meta-learning to co-evolve with system defenses \cite{goyal2023survey}.

\textbf{Threat roles and surfaces} vary in observability and access: white-box agents emulate insider threats with full model access; gray-box attackers observe intermediate features or metadata; black-box adversaries interact only with system inputs and outputs \cite{goyal2023survey,papernot2017practical}. Attack surfaces span semantic-aware jamming, backdoor insertion, knowledge poisoning, privacy leakage, and coordinated misinformation in multi-agent settings. A modular red-teaming framework should support diverse attacker profiles and allow composition of complex, multi-phase campaigns that reflect real-world threat evolution.

\textbf{Integrated evaluation} embeds red-teaming agents into training, adaptation, or runtime inference to reveal resilience under dynamic pressure. Defenses such as decoder switching, abstention, or knowledge re-synchronization can be stress-tested using runtime triggers like semantic mismatch, latent trust drift, or envelope violations \cite{meng2025securesemcom}. Beyond degrading performance, red-teaming enables \textit{semantic risk auditing}—a diagnostic process that identifies brittle input modalities, fragile concept classes, and cascading failure paths. These insights support the development of semantic risk budgets that quantify acceptable degradation bounds under adversarial stress, particularly for safety-critical applications such as autonomous driving, remote surgery, or multi-agent coordination.

Ultimately, red-teaming is not a replacement for theoretical analysis or benchmark testing but a necessary complement. By exposing emergent, cross-layer vulnerabilities that elude static analysis, red-teaming provides a pathway toward more trustworthy, resilient SemCom systems. Future work should prioritize open-source red-teaming toolkits tailored to SemCom, incorporating domain-specific artifacts such as latent codes, shared priors, and task-conditioned decoders. However, even the most sophisticated simulations must ultimately be validated under physical constraints, motivating real-world testbed deployments.

\subsection{Real-World Testbeds and Deployment Studies}
Simulation and red-teaming offer powerful abstractions for evaluating SemCom security. However, validating resilience under real-world constraints requires deployment-centric testbeds that expose the unpredictability of physical hardware, asynchronous control loops, and imperfect communication channels.

\textbf{Semantic observability} is central to effective deployment studies. Unlike conventional wireless testbeds that focus on throughput, delay, or error rates, SemCom evaluation requires introspection into latent code distributions, semantic drift, decoder disagreement, and knowledge desynchronization. Emerging 6G/O-RAN platforms \cite{bonati2021intelligence,polese2023understanding}, augmented with SDRs, xApps, and edge AI accelerators, provide partial support for this layered introspection. These platforms must be extended to monitor high-level behaviors such as task-level degradation under semantic mismatch and adversarial drift.

Testbeds expose \textbf{practical system constraints} that often go unnoticed in simulation. Knowledge re-synchronization mechanisms may fail under lossy control channels or when agents are asynchronously updated. Redundancy-based defenses, such as ensemble decoding or semantic voting, may conflict with stringent real-time latency constraints typical of edge environments. Practical issues such as hardware timing violations, adaptation delays, and resource contention often emerge as performance bottlenecks during deployment and must be explicitly profiled.

Beyond synthetic benchmarks, testbeds allow \textbf{cross-domain robustness evaluation} across realistic and heterogeneous settings, ranging from remote robotic control and telehealth to rural IoT deployments \cite{qiu2018can}. These domains introduce asymmetric vulnerabilities: low-power encoders at the edge may rely on powerful, semantically informed decoders in the cloud, resulting in one-sided failure modes when semantic codes are distorted or desynchronized. Edge–cloud heterogeneity, link asymmetry, and mobility further stress semantic security under real-world operating envelopes.


\begin{table*}[!t]
\centering
\caption{Deployment-Aware Evaluation Dimensions for Semantic Communication Security.}
\label{tab:evaluation-framework}
\begin{tabular}{|p{2.5cm}|p{3.5cm}|p{5cm}|p{5cm}|}
\hline
\textbf{Evaluation Goal} & \textbf{Security Objective} & \textbf{Evaluation Method} & \textbf{Representative Threats and Failure Modes} \\
\hline
\textbf{Semantic Robustness} & Meaning preservation and task utility under adversarial semantic perturbations & Semantic fidelity metrics, adversarial perturbation tests, semantic envelope violation rates & Knowledge misalignment, decoder drift, semantic corruption \\
\hline
\textbf{Semantic Leakage} & Privacy exposure from latent representations or shared knowledge & Mutual information analysis, inversion success rate, sensitive attribute recovery & Latent inversion, encoder leakage, cross-task information leakage \\
\hline
\textbf{Operational Resilience} & Tradeoffs between robustness, latency, and energy under adversarial and runtime constraints & Latency–robustness curves, energy per bit of meaning, graceful degradation tests & Time-critical failures, resource exhaustion, edge deployment stress \\
\hline
\textbf{Threat Adaptability} & System behavior under adaptive, multi-phase adversaries & Adaptive red-teaming agents, multi-stage and feedback-driven stress testing & Gray-box jammers, encoder poisoning, semantic desynchronization \\
\hline
\textbf{Deployment Robustness} & Resilience under real-world hardware, protocol, and update constraints & SDR-based testbeds, fault injection, runtime observability and monitoring & Semantic-aware jamming, asynchronous updates, decoder disagreement \\
\hline
\end{tabular}
\end{table*}


\textbf{Controlled fault injection} provides additional levers for testing adversarial resilience. SDR-based waveform injection can simulate semantic jamming at the physical layer. Compromised agents can be used to poison models or propagate misinformation through shared knowledge graphs. These setups further support fallback evaluations, including abstention, human-in-the-loop verification, and automated triggers for semantic anomalies.
To enable reproducible and modular evaluation, future efforts should prioritize open-source testbeds that integrate semantic communication pipelines, red-teaming agents, and runtime observability. Platforms such as Powder-RENEW \cite{powderrenew}, B5G Playground \cite{b5gplayground}, OpenAirInterface \cite{oai2023}, ARA \cite{ara2020testbed}, and RISE-6G \cite{rise6g2023} provide promising foundations for SemCom-aware security experimentation and system-level validation.

In summary, a comprehensive evaluation framework for SemCom security must integrate structured metrics (Section VI.A), dynamic threat simulation (Section VI.B), and real-world deployments. Table~\ref{tab:evaluation-framework} summarizes the key evaluation dimensions discussed in this section, highlighting metrics and methodologies for assessing SemCom security under adversarial and deployment-realistic conditions.
%, as summarized in Table \ref{tab:evaluation-framework}. Only by combining introspective, adversarial, and physical perspectives can we ensure that SemCom systems remain robust and trustworthy in practice.

% \section{Evaluation Frameworks for Semantic Communication Security}\label{sec:evaluation}
% Evaluating the security of SemCom systems requires fundamentally different methodologies than those used in traditional wireless or standalone AI settings. Unlike classical metrics that emphasize bit-level fidelity or model accuracy under independent and identically distributed (i.i.d.) inputs, SemCom systems operate across layers, where meaning is formed by the interplay between encoder-decoder pairs, channel characteristics, shared knowledge, and inference tasks. As such, robustness and utility must be assessed jointly and holistically, taking into account system constraints, attack surfaces, and task goals. 

% This section outlines the emerging principles, metrics, and experimental frameworks for evaluating secure SemCom systems, with emphasis on standardizing semantic robustness evaluation under constrained, adversarial, and deployment-realistic conditions. We begin by examining foundational evaluation metrics and benchmark needs for semantic security (A), followed by threat simulation and red-teaming approaches to probe practical vulnerabilities (B), and conclude with a discussion of real-world testbeds and deployment validation strategies (C).

% \subsection{Evaluation Metrics and Benchmarks}
% Despite significant progress in SemCom systems, the evaluation of their security remains insufficiently defined. Most existing studies assess performance using isolated task-level metrics, such as BLEU scores or classification accuracy, or rely on communication-centric indicators such as PSNR or bit error rate. While informative in limited contexts, these metrics do not capture the defining characteristics of secure SemCom: robustness under adversarial perturbations, dependence on shared knowledge and context, and operation under stringent latency, energy, and resource constraints. As a result, comparisons across designs are difficult, and deployment-relevant security guarantees remain elusive.

% To support reproducible, comparable, and system-level evaluation, semantic security must be assessed through a structured set of metrics that jointly reflect meaning preservation, adversarial resilience, and operational feasibility. We organize these metrics into four complementary categories.

% \textbf{Semantic utility} metrics form the foundation of SemCom evaluation. At their core is the question of whether the intended meaning is preserved under operational conditions. In task-driven settings, this is often measured through task accuracy, such as classification correctness or decision success. For language, vision, and multimodal communication, semantic similarity metrics including BLEU, ROUGE, CIDEr, or learned embedding-based scores such as CLIP similarity are commonly used to quantify reconstruction fidelity. In goal-directed or interactive systems, intent preservation becomes critical, requiring evaluation of whether downstream actions or inferred objectives align with the original communicative goal. In safety-critical deployments, abstention or fallback behavior must also be accounted for, as the ability to withhold decisions under low confidence can be as important as correctness itself. Importantly, semantic utility should be reported under both benign and adversarial conditions to expose robustness degradation rather than average-case performance.

% Beyond utility, \textbf{robustness and security metrics} are essential for characterizing resistance to semantic attacks. Rather than relying on classical $l_p$-norm–bounded perturbations, SemCom robustness must be defined with respect to adversarial budgets that reflect semantic corruption, channel power constraints, or poisoning intensity. Semantic robustness curves, which plot task utility against adversarial strength, provide a concise view of degradation behavior. Worst-case semantic distortion captures the maximum loss in utility under constrained attacks, offering a conservative security measure. At the representation level, latent code perturbability quantifies the sensitivity of semantic decoding to perturbations in learned embeddings. Privacy-oriented evaluation further requires measuring semantic leakage, such as the success of sensitive attribute inference or mutual information between latent representations and private data. These metrics reflect the fact that semantic security is as much about limiting inference as it is about preserving correctness.

% Because semantic defenses operate within real systems, \textbf{operating envelope metrics} are equally critical. Security mechanisms inevitably interact with latency, throughput, and energy budgets, and these interactions must be explicitly evaluated. Latency–robustness tradeoffs reveal how defensive actions affect deadline miss rates or tail latency. Throughput versus semantic fidelity captures how robust encoding and retransmission policies scale under attack or interference. Energy per bit of meaning provides a unified measure of communication and computation cost relative to semantic utility, particularly relevant for edge and IoT deployments. Finally, adversarial envelope violation rates quantify how often system performance falls below application-specific semantic thresholds under constrained attacks. Visualizing these relationships as operating envelopes, for example task accuracy as a function of SNR and adversarial power, enables system designers to reason about acceptable operating regions rather than single-point performance.

% Despite these emerging principles, \textbf{benchmarking practice} in secure SemCom remains fragmented. Most evaluations rely on isolated datasets such as CIFAR-10 or COCO with offline corruption models, neglecting over-the-air effects, multi-agent interaction, and adaptive adversaries. There is currently no public benchmark suite designed specifically for semantic communication security that incorporates semantic attacks, cross-layer faults, or dynamic knowledge states. Moreover, many simulation environments abstract away realistic wireless behavior, adversarial scheduling, and evolving knowledge graphs, limiting their relevance to deployment.

% Addressing these gaps requires the development of SemCom-native benchmarks that span image, speech, and text modalities with explicit semantic goals and threat scenarios. Such benchmarks should integrate channel simulators capable of modeling adversarial fading, semantic jamming, and protocol-aware perturbations, alongside standardized evaluation pipelines that jointly measure semantic fidelity, robustness, delay, and resource consumption. Establishing these benchmarks is a prerequisite for meaningful comparison across defense strategies and for translating semantic security research into deployable systems.


% \subsection{Threat Simulation and Red-Teaming}
% While theoretical threat models and benchmark-driven evaluations have laid the foundation for assessing semantic communication security, they often fall short of capturing the complexity and adaptiveness of real-world adversaries. SemCom systems are exposed to a broad range of vulnerabilities across model, channel, knowledge, and network layers—surfaces that can be exploited individually or in combination. To evaluate system robustness against such multifaceted threats, \textbf{red-teaming} provides a complementary methodology: it simulates intelligent, adversarial agents capable of probing, manipulating, and subverting the semantic pipeline through dynamic, feedback-driven strategies.

% In contrast to static perturbation models, \textbf{adaptive adversarial simulation} reflects a more realistic attack scenario in which the adversary observes system responses and adjusts its tactics accordingly. For example, semantic jammers can be trained to react to partial feedback such as task confidence or retransmission frequency, evolving interference patterns that target vulnerable aspects of the receiver’s inference process. Similarly, gray-box adversaries may query the encoder-decoder interface to extract latent representations, reconstruct decision boundaries, or trigger semantic misinterpretation. These attacks can also be composed across layers: subtle encoder poisoning, coupled with channel-level perturbations and knowledge-base desynchronization, can lead to emergent failures that are hard to detect or attribute. Implementing such red-teaming agents requires the use of reinforcement learning, meta-learned perturbation generators, or adversarial co-training frameworks that co-evolve with the system being tested.

% Effective red-teaming must account for diverse \textbf{threat roles and access levels}. White-box adversaries simulate insider threats or compromised devices with access to model weights and training data. Gray-box attackers reflect partially informed actors who observe intermediate outputs, metadata, or channel state. Black-box adversaries operate solely through input–output interaction, emulating external or over-the-air threats in open deployments. Across these roles, adversaries may target different components: implanting backdoors in model training, performing inference-time evasion, injecting semantic-aware jamming at the physical layer, corrupting or desynchronizing shared knowledge, or propagating misinformation in multi-agent settings. An effective red-teaming framework should allow modular composition of these capabilities and support simulation across a range of configurations, enabling defenders to evaluate not just isolated modules but the system’s layered defenses and fallback strategies in the face of coordinated threats.

% For threat simulation to inform system design and deployment, it must be \textbf{integrated into evaluation pipelines}. This includes injecting adversarial behavior during training, adaptation, or inference, and monitoring the resulting impact on semantic utility, operating envelope violations, and decision confidence. Defenses that respond dynamically—such as abstention, decoder switching, or knowledge re-synchronization—can be evaluated under conditions where attacks adapt in real time. Semantic mismatch rates, disagreement between modules, or observed trust drift can be used as runtime triggers for activating these responses. Red-teaming agents can therefore serve not only as evaluators but as part of a closed-loop simulation ecosystem in which robustness is assessed under dynamic, adversarial feedback.

% Beyond performance degradation, red-teaming also enables \textbf{semantic risk auditing}, a diagnostic process that aims to identify and characterize systemic fragilities. For instance, it can help determine which classes of concepts, tasks, or input modalities are most vulnerable to distortion or leakage, or which combinations of model, channel, and knowledge configurations lead to the most brittle behavior. In safety-critical applications such as autonomous driving or remote control, these insights can guide the formulation of semantic risk budgets—quantitative guarantees on acceptable levels of degradation under known attack budgets. Red-teaming can then be used to validate whether system behavior remains within these contractual bounds, even in the presence of sophisticated adversaries.

% Ultimately, red-teaming is not a replacement for theoretical analysis or static benchmarks, but a necessary complement. It brings an adversarial lens to SemCom evaluation, exposing the subtle interactions and emergent behaviors that arise from AI-native design, layered architecture, and dynamic adaptation. To support reproducibility and progress in this area, future efforts should focus on developing open-source red-teaming frameworks tailored to SemCom pipelines, incorporating artifacts such as latent semantic codes, shared knowledge graphs, and end-to-end task fidelity. Such frameworks will be critical for building secure, adaptive, and trustworthy semantic communication systems.

% \subsection{Real-World Testbeds and Deployment Studies}
% While simulation and red-teaming offer powerful abstractions for evaluating SemCom security, translating these findings into real-world reliability requires deployment-centric validation. Semantic communication systems, with their AI-native encoding, cross-layer interactions, and context-dependent reasoning, behave differently when exposed to the uncertainties, imperfections, and constraints of operational environments. Testbed deployment serves as the bridge between theory and practice, offering a sandbox to evaluate robustness, adaptivity, and system-level behavior under realistic conditions.

% A key requirement for deployment studies is semantic observability across layers. Traditional wireless testbeds focus on physical- or network-layer metrics—throughput, delay, packet error rates. In contrast, semantic communication demands instrumentation capable of tracking high-level representations: latent code distributions, semantic task fidelity, decoder alignment, and knowledge synchronization. Emerging 6G and O-RAN platforms provide partial support for such semantic introspection, especially when integrated with software-defined radios (SDRs), edge AI accelerators, and flexible radio access control. Experimental setups must extend these capabilities to monitor semantic drift over time, detect context mismatches, and correlate adversarial perturbations with task-level degradation.

% Real-world testbeds also reveal deployment challenges hidden in simulation, including hardware constraints, system-level timing violations, and adaptation latencies. For example, knowledge resynchronization mechanisms that work well in simulation may be infeasible when distributed agents have mismatched updates or lossy control channels. Similarly, redundancy-based defenses such as ensemble decoding or semantic voting may conflict with latency budgets in edge environments. Deployment studies expose these conflicts, allowing designers to tune tradeoffs between robustness and resource consumption in context-sensitive ways.

% Testbeds enable cross-domain evaluation, where robustness is assessed across multiple application settings—autonomous driving, remote control, edge intelligence, or telehealth. This allows researchers to test whether proposed semantic encodings, certification methods, or fallback strategies generalize beyond synthetic datasets and single-task benchmarks. In particular, edge–cloud heterogeneity and link asymmetry—such as constrained encoders in rural IoT and powerful decoders at aggregation points—create asymmetrical vulnerabilities that can only be evaluated under realistic communication and computational conditions.

% Moreover, testbed deployments support security-focused fault injection, enabling controlled testing of physical-layer jamming, adversarial inputs, or compromised agents. For instance, adversarial waveforms can be injected over-the-air using SDRs to assess semantic jamming resilience. Model poisoning or desynchronized knowledge bases can be introduced to emulate compromised devices. These experiments make it possible to validate fallback mechanisms such as abstention, re-synchronization, or human-in-the-loop verification under actual operational stress, rather than abstract assumptions.

% To support reproducible research and standardized evaluations, there is a growing need for open-source SemCom testbed platforms that integrate semantic encoders/decoders, adversarial modules, and real-time instrumentation. These platforms should provide modular support for tuning channel conditions, injecting semantic-aware perturbations, and measuring end-to-end task reliability. Initiatives such as the ARA rural testbed, O-RAN-based xApp platforms, or edge AI inference over programmable radio networks represent promising foundations for such SemCom-centric evaluations.

% In summary, real-world testbeds play a critical role in closing the gap between algorithmic robustness and system-level trust. By enabling reproducible, configurable, and domain-relevant experimentation, they ensure that semantic security mechanisms do not remain theoretical constructs but evolve into deployable defenses that can withstand the unpredictability of real-world environments.
